Sparse-VQ Transformer: An FFN-Free Framework with Vector Quantization for Enhanced Time Series Forecasting

Time series analysis is vital for numerous applications, and transformers have become increasingly prominent in this domain. Leading methods customize the transformer architecture from NLP and CV, utilizing a patching technique to convert continuous signals into segments. Yet, time series data are uniquely challenging due to significant distribution shifts and intrinsic noise levels. To address these two challenges,we introduce the Sparse Vector Quantized FFN-Free Transformer (Sparse-VQ). Our methodology capitalizes on a sparse vector quantization technique coupled with Reverse Instance Normalization (RevIN) to reduce noise impact and capture sufficient statistics for forecasting, serving as an alternative to the Feed-Forward layer (FFN) in the transformer architecture. Our FFN-free approach trims the parameter count, enhancing computational efficiency and reducing overfitting. Through evaluations across ten benchmark datasets, including the newly introduced CAISO dataset, Sparse-VQ surpasses leading models with a 7.84% and 4.17% decrease in MAE for univariate and multivariate time series forecasting, respectively. Moreover, it can be seamlessly integrated with existing transformer-based models to elevate their performance.

==> sections/2_related_work.tex <==
\section{Related Work}\label{sec_related_works}

%{\color{blue}

\subsection{Time-series Forecasting}

Temporal variation modeling is a prominent issue in time series analysis and has been extensively investigated with numerous methods been proposed to achieve accurate long-term time series forecasting.

Early studies typically employed traditional statistical methods or machine learning techniques, such as ARIMA (Anderson \& Kendall, 1976) \cite{box_arima2}, Holt-Winter (Hyndman \& Athanasopoulos, 2018) \cite{Holt-Winter18}, DeepAR (Salinas et al., 2020)\cite{DBLP:journals/corr/FlunkertSG17-deepAR} and Prophet (Taylor \& Letham, 2018) \cite{Taylor2018ForecastingAS}. With the rise of deep learning, researchers have turned their attention to more robust and complex neural networks for time series modeling, including TCN (Bai et al., 2018) \cite{TCN}, LSTM (Hochreiter et al., 1997)\cite{hochreiter_long_1997_lstm}. Specifically, N-BEATS (Oreshkin et al., 2019) \cite{nbeats} designed an interpretable layer by encouraging the model to learn trend, seasonality explicitly, and residual components, which shows superior performance on the M4 competition dataset; Dlinear (Zeng et al., 2022)\cite{Dlinear} employs a simple linear layer, while TimesNet (Wu et al. 2023) \cite{TIMESNET} extends the analysis of temporal variations into the 2D space enabling to discover the multi-periodicity adaptively and extract the complex temporal variations. 

Among these, the Transformer (Vaswani et al., 2017) ~\cite{attention_is_all_you_need} and its subsequent adaptations have demonstrated significant success in long sequence modelling tasks, including time series forecasting.  Informer (Zhou et al., 2021) \cite{haoyietal-informer-2021} proposes a ProbSparse self-attention mechanism and distilling operation to address the quadratic complexity of the Transformer, while Reformer (Kitaev et al., 2020)\cite{KitaevKL20-reformer} replaces dot-product attention by using locality-sensitive hashing and improves its complexity, resulting in significant performance improvements. Subsequently, Autoformer (Wu et al. 2021) \cite{Autoformer} designs an efficient auto-correlation mechanism to discover and aggregate information at the series level; FiLM (Zhou
et al., 2022) \cite{zhou2022film} design a Frequency improved Legendre Memory model applying Legendre polynomial projections to approximate historical information, while FEDformer 
et al., 2022) \cite{FedFormer} proposes an attention mechanism with low-rank approximation in frequency and a mixture of experts decomposition to control the distribution shifting. Additionally, Pyraformer (Liu et al., 2022) \cite{liu2022pyraformer} designs pyramidal attention to effectively describe short and long temporal dependencies with low time and space complexity and patchTST (Nie et al., 2023) \cite{patchTST} embeds the whole time series of each variate independently into tokens to enlarge local receptive field. Recently, FPT (Zhou
et al., 2022) \cite{zhou2023onefitsall} leverages pretrained language or CV models for time series analysis firstly and achieves excellent performance in all main time series analysis tasks. Overall, the Transformer architecture is widely regarded as one of the most effective and promising approaches for MTS forecasting (wen et al., 2022\cite{Wen2022transformers}; shao et al., 2023 \cite{Shao2023exploring}).


\subsection{Distribution shift} 

Although various models above make breakthroughs in time-series forecasting, they often encounter challenges when dealing with non-stationary time-series data, where the distribution of the data changes over time. To address this issue, domain adaptation (Tzeng et al., 2017 \cite{Tzeng17Domain_Adaptation}; Ganin et al., 2016 \cite{Ganin16domain_adaptation}; Wang et al., 2018 \cite{Wang18Domain_Adaptation}) and domain generalization (Wang et al., 2021 \cite{Wang2021GeneralizingTU}; Li et al., 2018\cite{Li18DomainGeneralization}; Muandet et al., 2013 \cite{pmlr-v28-muandet13}; Lu et al., 2022 \cite{Lu2022DomaininvariantFE}) approaches are commonly employed to mitigate the distribution shift. Domain adaptation algorithms aim to reduce the distribution gap between the source and target domains, while domain generalization algorithms solely rely on the source domain and aim to generalize to the target domain. 
However, defining a domain becomes challenging in the context of non-stationary time series, as the data distribution shifts over time. Recently, Du et al. (Du et al., 2021) proposed the use of Adaptive RNNs to address the distribution shift issues in non-stationary time-series data,  characterizing the distribution information by dividing the training data into periods and then matches the distributions of these identified periods to generalize the model. RevIN (Kim et al. 2022) \cite{reversible} utilizes a generally applicable normalization-and-denormalization method with learnable affine transformation to address the distribution shift problem. DIVERSIFY (Lu et al. 2023) \cite{lu2023outofdistribution} trys to learn the out of-distribution (OOD) representation on dynamic distributions of times series and then bridges the gap between these latent distributions.



\subsection{Vector Quantization}

Vector quantization (VQ) is a widely used compression technique in signal and image processing, which aims to learn a discrete latent representation by clustering multidimensional data into a finite set of representations. VQ-VAE (Van Den Oord et al., 2017)\cite{VQVAE} proposes to combine the VQ strategy with a variational autoencoder. There are two key differences between this approach and VAEs: first, the encoder network produces discrete codes instead of continuous ones to obtain a compressed discrete latent space; second, the prior is learned rather than being static; which make it capable of modelling very long term dependencies. SoundStream(Zeghidour et al., 2021) \cite{residualVQ} proposes the residual VQ and employs multiple vector quantizers to iteratively quantize the residuals of the waveform.VQ has also been combined with adversarial learning to synthesize high-resolution images, for example, VQGAN (Esser et al., 2021)\cite{VQGAN}. Subsequently, ViT-VQGAN(Yu et al., 2022)\cite{VQGAN_use_cosine_sim} propose to reduce the dimensionality of the codebook and l2-normalize the codebook and TE-VQGAN(Shin et al., 2023)\cite{orthogonal} incorporate a regularization term into the loss function to enforce orthogonality among the codebook embeddings. Considering veiwing time series as several discrete tokens may be potentially useful, our framework uniquely leverages VQ to enhance the capabilities of transformers in time series forecasting.

%end color blue
%}

%\subsection{Modeling both local and global context} 
%The receptive field of a CNN is restricted by the size of the convolutional kernel, making it more suitable for local information modeling. On the other hand, Self-Attention (SA) computes attention weights for each position with respect to all positions, effectively taking into account the relationships between each point. Consequently, SA appears more appropriate for global modeling. However, point-wise representation might inhibit the model from summarizing a long historical signal, and long input SA may be prone to overfitting.

%In order to capture both global and local information and model more granular information effectively, an increasing number of research works have adopted a hybrid approach by combining these two structures. MUSE~\cite{zhao2019muse} investigates the integration of convolution and self-attention mechanisms to enable the learning of sequence representations that incorporate multiple scales. T2VLAD~\cite{WangZ021} designs an efficient global-local alignment method to search relevant video contents based on natural language descriptions. VOLO~\cite{yuan2022volo} not only focuses on global modeling at a coarse level, but also efficiently encodes finer-level features and contexts into token. In the field of time series forecasting, MICN~\cite{wang2023micn} proposes a local-global structure to implement information aggregation and long-term dependency modeling for time series, but both local information and global information are obtained through convolutional neural networks (CNNs), and two structures are composed in a serial manner.



% }


% \section{Time Series Representation in Legendre-Fourier Domain} \label{sec:theoretical}

% \subsection{Legendre Projection}
%  Given an input sequence, the function approximation problem aims to approximate the cumulative history at every time $t$. Using Legendre Polynomials projection, we can project a prolonged sequence of data onto a subspace of bounded dimension, leading to compression, or feature representation, for evolving historical data. Formally, given a smooth function $f$ observed online, we aim to maintain a fixed size compressed representation of its history $f(x)_{[t-\theta,t]}$, where $\theta$ specifies the window size. At every time point $t$, the approximation function $g^{(t)}(x)$ is defined with respect to the measure $\mu^{(t)} =\frac{1}{\theta}\mathbbm{I}_{[t-\theta,t]}(x)$. In this paper, we use Legendre Polynomials of degree at most $N-1$ to build the function $g^{(t)}(x)$, i.e.
%   \begin{align}
%   g^{(t)}(x)=\sum_{n=1}^N c_{n}(t) P_{n}\left(\frac{2(x-t)}{\theta}+1\right), \label{eq:1}
%  \end{align}
%  where $P_n(\cdot)$ is the $n$-th order Legendre Polynomials. Coefficients $c_{n}(t)$ are captured by the following dynamic equation:
% \begin{align}%\notag
%  \frac{d}{d t} c(t) &=-\frac{1}{\theta} A c(t)+\frac{1}{\theta} B f(t).
% \end{align}
% where the definition of $A$ and $B$ can be found in~\cite{LMU}. Using Legendre Polynomials as a basis allows us to accurately approximate smooth functions, as indicated by the following theorem.

% \begin{theorem} [\it Similar to Proposition 6 in \cite{Hippo}]
%  If $f(x)$ is $L$-Lipschitz, then $\|f_{[t-\theta,t]}(x)-g^{(t)}(x)\|_{\mu^{(t)}}\le \mathcal{O}(\theta L/\sqrt{N})$. Moreover, if $f(x)$ has $k$-th order bounded derivatives, we have $\|f_{[t-\theta,t]}(x)-g^{(t)}(x)\|_{\mu^{(t)}}\le \mathcal{O}(\theta^kN^{-k+1/2})$.
% \end{theorem}
% According to Theorem 1, without any surprise, the larger the number of Legendre Polynomials basis, the more accurate the approximation will be, which unfortunately may lead to the overfitting of noisy signals in history. As shown in Section \ref{sec_exp}, directly feeding deep learning modules, such as MLP, RNN, and vanilla Attention without modification, with the above features will not yield state-of-the-art performance, primarily due to the noisy signals in history. That is why we introduce, in the following subsection, a Frequency Enhanced Layer with Fourier transforms for feature selection.  

% %The above theorem implies that if we pick proper $N$, the $g^(t)(x)$ function will be good enough to memorize the function $f_{[t-\theta, t]}(x)$ and we could use coefficient of $c_n(t)$ of $g^{(t)}(x)$ as the proper representation for the time series.

% Before we close this subsection, we note that unlike~\cite{S4}, a fixed window size is used for function approximation and feature extraction. This is because a longer history of data may lead to a larger accumulation of noises from history. To make it precise, we consider an auto-regressive setting with random noise. Let $\{x_t\}\in \mathbbm{R}^d$ be the time sequence with $x_{t+1} = Ax_t + b + \epsilon_t$ for $t=1,2,...$, where $A\in\mathbbm{R}^{d\times d}$, $b \in \mathbbm{R}^d$, and $\epsilon_t\in\mathbbm{R}^{d}$ is random noise sampled from $N(0, {\sigma^2 I})$. As indicated by the following theorem, given $x_t$, the noise will accumulate in $x_{t-\theta}$ over time at the rate of $\sqrt{\theta}$, where $\theta$ is the window size.

% \begin{theorem}
% Let $A$ be an unitary matrix and $\epsilon_t$ be $\sigma^2$-subgaussian random noise.  We have $x_{t} = A^{\theta}x_{t-\theta} + \sum_{i=1}^{\theta-1}A^{i}b + \mathcal{O}(\sigma \sqrt{\theta})$.
% \end{theorem}
 

% \subsection{Fourier Transform}
% % {\color{red} (TODO: to be finished??)} \Xue{(Sure, will try to finish it today or tomorrow...)}
% % $$x_{t+1} = Ax_t + b =  (A^{n-1}+A^{n-2}+...+I)bx_0 + O(b)$$
% % $$x_{t+1} = Ax_t + b +\epsilon_t = (A^{n-1}+A^{n-2}+...+I)bx_0 +O(b) + \sum \epsilon_t = O(\sqrt{T}\log T)$$
% Because white noise has a completely flat power spectrum, it is commonly believed that the time series data enjoys a particular spectral bias, which is not generally randomly distributed in the whole spectrum.
% % \Xue{(may need some references)}
% Due to the stochastic transition environment, the real output trajectories of the forecasting task contain large volatilization and people usually only predict the mean path of them. The relatively more smooth solutions thus are preferred. According to Eq.~\eqref{eq:1},  the approximation function $g^{(t)}(x)$ can be stabilized via smoothing the coefficients $c_n(t)$ in both $t$ and $n$. This observation helps us design an efficient data-driven way to tune the coefficients $c_n(t)$. As smoothing in $n$ can be simply implemented via multiplying learnable scalars to each channel, we mainly discuss smoothing $c_n(t)$ in $t$ via Fourier transformation. The spectral bias implies the spectrum of $c_n(t)$ mainly locates in the low-frequency regime and has weak signal strength in the high-frequency regime. To simplify our analysis, let us assume the Fourier coefficients of $c_{n}(t)$ as $a_{n}(t)$. Per spectral bias, we assume that there exists a $s, a_{\min}>0$, such that for all $n$ we have $t> s$, $|a_{n}(t)|\le a_{\min}$. An idea to sample coefficients is to keep the first $k$ dimensions and randomly sample the remaining dimensions instead of the fully random sampling strategy. We characterize the approximation quality via the following theorem:

% \begin{theorem}
% \label{thm_Fourier} 
% Let $A\in\mathbbm{R}^{d\times n}$ be the Fourier coefficients matrix of an input matrix $X\in\mathbbm{R}^{d\times n}$, and $\mu(A)$, the coherence measure of matrix $A$, is $\Omega(k/n)$. We assume there exist $s$ and  a positive $ a_{\min}$ such that the elements in last $d-s$ columns of $A$ is smaller than $a_{\min}$. If we keep the first $s$ columns selected and randomly choose $\mathcal{O}(k^2/\epsilon^2 - s)$ columns from the remaining parts, with high probability
% \[
%     \|A - P(A)\|_F \leq \mathcal{O}\left[(1 + \epsilon)a_{\min}\cdot\sqrt{(n-s)d}\right],
% \]
% where  $P(A)$ denotes the matrix projecting $A$ onto the column selected column space.
% \end{theorem}
% Theorem~\ref{thm_Fourier} implies that when $a_{\min}$ is small enough, the selected space can be considered almost the same as the original one.

==> tables/full_bench_multi.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). A lower MSE indicates better performance. All experiments are repeated 5 times.}\vspace{-1mm}
\scalebox{0.60}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
                        & 192 & \textbf{0.222} & \textbf{0.296} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
                        & 720 & \textbf{0.371} & \textbf{0.389} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} &96  &\textbf{0.154}  &\textbf{0.267}  &0.183 &0.297 &0.201  &0.317 &0.304 &0.405 &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.195 &0.308 &0.222  &0.334 &0.313 &0.413 &0.296 &0.386  &0.266 &0.368  &0.348  &0.433    \\
                        & 336 & \textbf{0.188} & \textbf{0.283} &0.212 &0.313 &0.231 &0.338 &0.290 &0.381 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
                        & 720 & 0.236 & \textbf{0.332} &\textbf{0.231} &0.343 &0.254  &0.361 &0.262 &0.344 &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & \textbf{0.086} & \textbf{0.204} &0.139 &0.276 &0.197  &0.323 &1.292 &0.849 &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
                        & 192 & \textbf{0.188} & \textbf{0.292} &0.256 &0.369 &0.300  &0.369 &1.631 &0.968 &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
                        & 336 & \textbf{0.356} & \textbf{0.433} &0.426 &0.464 &0.509  &0.524 &2.225 &1.145 &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
                        & 720 & \textbf{0.727} & \textbf{0.669} &1.090 &0.800 &1.447  &0.941 &2.521 &1.245 &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &\textbf{0.416}& \textbf{0.294} &0.562 &0.349 &0.613  &0.388 &0.824 &0.514 &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
                        & 192 & \textbf{0.408} & \textbf{0.288} &0.562 &0.346 &0.616&0.382 &1.106 &0.672 &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
                        & 336 & \textbf{0.425} & \textbf{0.298} &0.570 &0.323 &0.622  &0.337 &1.084 &0.627 &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
                        & 720 & \textbf{0.520} &\textbf{0.353} &0.596 &0.368 &0.660  &0.408 &1.536 &0.845 &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.199} & \textbf{0.262} &0.217  &0.296  &0.266  &0.336 &0.406 &0.444 &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
                        & 192 & \textbf{0.228} & \textbf{0.288} &0.276  &0.336  &0.307  &0.367 &0.525 &0.527 &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
                        & 336 &\textbf{0.267} &\textbf{0.323} & 0.339  &0.380  &0.359  &0.395 &0.531 &0.539 &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
                        & 720 &\textbf{0.319} & \textbf{0.361} &0.403  &0.428 &0.578 &0.578 &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & \textbf{1.970} & \textbf{0.875} &2.203  &0.963  &3.483 &1.287 &4.631 &1.484 &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
                        & 36 & \textbf{1.982} & \textbf{0.859} &2.272  &0.976  &3.103  &1.148 &4.123 &1.348 &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
                        & 48 & \textbf{1.868} & \textbf{0.896} &2.209  &0.981  &2.669  &1.085 &4.066 &1.36 &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
                        & 60 & \textbf{2.057} & \textbf{0.929} &2.545  &1.061  &2.770  &1.125 &4.278 &1.41 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/full_bench_uni.tex <==
\begin{table*}[h]
% \begin{adjustwidth}{-1.5in}{-1in}
\centering
%\begin{small}
\caption{Univariate long-term forecasting results on six datasets with various input length and prediction horizon $O \in \{96,192,336,720\}$. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.60}{
\begin{tabular}{c|c|cccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.065 &\textbf{0.189}  &\textbf{0.063} &0.189 & 0.065 & 0.189 &0.153 &0.318 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.094} & \textbf{0.233} &0.102 &0.245 & 0.118 & 0.256 &0.183 &0.350 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.124} & \textbf{0.274} &0.130 &0.279 & 0.154 & 0.305 &0.204 & 0.367 &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.173} & \textbf{0.323} &0.178 &0.325 & 0.182 &0.335 &0.482 &0.567  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
& 96  & \textbf{0.154} & \textbf{0.247} &0.253 &0.370  &0.341 &0.438 &0.351 &0.452 & 0.484& 0.538 &0.288& 0.393& 0.274 & 0.379   \\
& 192 & \textbf{0.166} & \textbf{0.258} &0.282 &0.386 &0.345 &0.428 &0.373 &0.455 & 0.557& 0.558 &0.432 & 0.483 & 0.304 &0.402   \\
& 336 & \textbf{0.188} & \textbf{0.283} &0.346 &0.431 &0.406 &0.470 &0.408 &0.477 & 0.636& 0.613 &0.430 &0.483 & 0.370 &0.448  \\
& 720 & \textbf{0.249} & \textbf{0.341} &0.422 &0.484 &0.565 &0.581 &0.472 &0.517 & 0.819& 0.682 &0.491 &0.531 & 0.460 &0.511   \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
&96  & \textbf{0.110} & \textbf{0.259} &0.131 &0.284 & 0.241 & 0.387 &0.344 &0.482  & 0.591  &0.615  &0.237 &0.377  &0.298  &0.444    \\
& 192 & \textbf{0.207} & \textbf{0.352} &0.277 &0.420 &0.300  &0.369 &0.362 &0.494  &1.183   &0.912 &0.738  &0.619  &0.777  & 0.719   \\
& 336 & \textbf{0.327} & \textbf{0.461} &0.426 &0.511 &0.509  &0.524 &0.499 &0.594  &1.367  &0.984  &2.018  &1.070  &1.832  &1.128     \\
& 720 & \textbf{0.811} & \textbf{0.708} &1.162 &0.832 &1.260  &0.867 &0.552 & 0.614 &1.872  &1.072  &2.405  &1.175  &1.203  &0.956     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  & \textbf{0.144} & \textbf{0.215} &0.170 &0.263  &0.246 &0.346 &0.194 &0.290 & 0.257 & 0.353 &0.226 &0.317 &  0.313 & 0.383\\
& 192 & \textbf{0.120} & \textbf{0.199} &0.173 &0.265 &0.266 &0.370 &0.172 &0.272 & 0.299 & 0.376 &0.314 &0.408 & 0.386 & 0.453\\
& 336 & \textbf{0.128} & \textbf{0.212} &0.178 &0.266 &0.263 &0.371 &0.178 &0.278 & 0.312 & 0.387 &0.387 &0.453 & 0.423 & 0.468\\
& 720 & \textbf{0.153} & \textbf{0.252} &0.187 &0.286 &0.269 &0.372 &0.263 &0.386 & 0.366 & 0.436 &0.491 &0.437 & 0.378 & 0.433\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}}
& 96  & \textbf{0.0012} & \textbf{0.026} & 0.0035 & 0.046 & 0.011 &0.081 &0.0061 &0.065 & 0.0038 & 0.044 & 0.0046 &0.052 & 0.012 & 0.087 \\
& 192 & \textbf{0.0014}& \textbf{0.029}&0.0054 &0.059 &0.0075 &0.067 &0.0067 &0.067 & 0.0023 & 0.040 &0.0056 & 0.060 & 0.0098 & 0.079  \\
& 336 & \textbf{0.0015} & \textbf{0.030} &0.0041 &0.050 &0.0063 &0.062 &0.0025 &0.0381 & 0.0041 & 0.049 &0.0060 &0.054& 0.0050 & 0.059 \\
& 720 & \textbf{0.0022} & \textbf{0.037} &0.015 &0.091 &0.0085 &0.070 &0.0074 &0.0736 & 0.0031 & 0.042 &0.0071 &0.063& 0.0041 & 0.049 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & \textbf{0.629} & \textbf{0.538} &0.693 &0.629 &0.948 &0.732 &0.866 &0.584 & 5.282 &2.050 &3.607 & 1.662 & 3.838 & 1.720  \\
& 36 & \textbf{0.444} & \textbf{0.481} &0.554 &0.604 &0.634 &0.650 &0.622 &0.532 & 4.554 &1.916 &2.407 & 1.363 & 2.934 & 1.520 \\
& 48 & \textbf{0.557} & \textbf{0.584} &0.699 &0.696 &0.791 &0.752 &0.813 &0.679 & 4.273 &1.846 &3.106 & 1.575 & 3.754 & 1.749\\
& 60 & \textbf{0.641} & \textbf{0.644} &0.828 &0.770 &0.874 &0.797 &0.931 &0.747 & 5.214 &2.057 &3.698 & 1.733 & 4.162 & 1.847\\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-large}
\vskip -0.10in
% \end{adjustwidth}
%\end{small}tab:multi-benchmarks
\end{table*}


==> tables/ks_test_small.tex <==

\begin{table}[h]
%\setlength{\uppercaptionskip}{0.pt}
%\setlength{\belowcaptionskip}{-0.pt}
%\vskip 0.15in
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{P-values of Kolmogrov-Smirnov test of different Transformer models for long-term forecasting output on ETTm1 and ETTm2 dataset. Larger value indicates the hypothesis (the input sequence and forecasting output come from the same distribution) is less likely to be rejected. The largest results are highlighted.}
\begin{small}
% \begin{sc}
\vskip 0.05in
\scalebox{0.80}{
\begin{tabular}{c|c|cccccc}
\toprule
\multicolumn{2}{c|}{Methods}&Transformer&Informer&Autoformer&FEDformer&FiLM&True\\ %&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 
& 96 & 0.0090 & 0.0055&0.020 & \textbf{0.048} & 0.016& {0.023} \\
& 192 & 0.0052 & 0.0029&0.015 & \textbf{0.028} & 0.0123& {0.013} \\
& 336 & 0.0022 & 0.0019&0.012 & \textbf{0.015} & 0.0046& {0.010} \\
% & 720 & 0.0023 & 0.0016 & \textbf{0.014} & \textbf{0.0036} \\
& 720 & 0.0023 & 0.0016&0.008 & \textbf{0.014} & 0.0024& {0.004} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
% & 48 & 0.454 & & 0.366 & & 0.476 & & 0.356 \\
& 96 & 0.0012 & 0.0008& \textbf{0.079} &{0.071} & 0.022 & {0.087} \\%& \textbf{0.379} & \textbf{0.419}\\
& 192 & 0.0011 & 0.0006& \textbf{0.047} &{0.045}  &0.020 & {0.060} \\%& \textbf{0.426} & \textbf{0.441}\\
% & 288 & 0.634 & & 0.430 & & 0.571 & & 0.379 \\
& 336 & 0.0005 & 0.00009& 0.027 &\textbf{0.028} &0.012 & {0.042} \\%& \textbf{0.445} & \textbf{0.459}\\
% & 672 & 0.606 & & 0.528 & & 0.544 & & 0.501\\
& 720 & 0.0008& 0.0002& \textbf{0.023} & {0.021} &0.0081 & {0.023} \\
% \multicolumn{2}{c|}{Count}& 0 & 0 & 3 & 5 & 7& NA \\
%& \textbf{0.543} & \textbf{0.490}\\
%& -96 & 0.0012 & 0.0009 & 0.0001 & 0.0037 & \textbf{0.039} & \textbf{0.012} \\
\bottomrule
\end{tabular}
}
\label{tab:KStest_small}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}




==> tables/tab_LPU_boosting.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
% \begin{wraptable}

% \begin{wraptable}[12]{r}{0.7\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Boosting effect of LPU layer for common deep learning backbones: MLP, LSTM, CNN and Attention.`+` indicates degraded performance.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
%\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEL}&\multicolumn{2}{c|}{MLP}&\multicolumn{2}{c|}{LSTM}&\multicolumn{2}{c|}{lagged-LSTM}&\multicolumn{2}{c|}{CNN}&\multicolumn{2}{c}{Attention}\\
\midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\multicolumn{2}{c|}{Compare} & LPU  & Linear& LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030}  & +38\%   & 0.034  & +8.0\%  & 0.049 & +73\% & 0.093 & -21\% & 0.116   & -50\%   & 0.243  & -81\% \\
& 192  &\textbf{0.047} & +9.5\% & 0.049  & +30\%  & 0.174 & +32\% & 0.331 & -48\% & 0.101   & +20\%    & 0.387  & -86\% \\
& 336 & \textbf{0.063} & +5.8\% & 0.061  & +64\%  & 0.119 & +84\% & 0.214 & -19\% & 0.122   & +25\%    & 1.652  & +12\% \\
& 720 &\textbf{0.081} & +1.4\%  & 0.082  & +62\%  & 0.184 & +32\% & 0.303 & -6.5\%  & 0.108   & +13\%    & 4.782  & -61\% \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
% &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

&96  &\textbf{0.213}  & +136\%  & 0.431  & +121\%   & 0.291 & +55.6\% & 0.739 & -33\% & 0.310  & +43\%  & 0.805 & +23\% \\%&--& --
& 192 &\textbf{0.268} & +32\%   & 0.291 & +239\%   & 0.353  & +17\% & 0.535 & +15\% & 0.380  & +12\%  & 0.938 & +14\% \\%&--& --  \\
& 336 & \textbf{0.307}& +0.1\%  & 0.296 & +235\%   & 0.436  & -6.7\% & 0.517 & +23\% & 0.359  & +29\% & 2.043 & -54\% & \\%&--& -- \\
& 720 & \textbf{0.321}& +37\%   & 0.339 & +196\%   & 0.636  & -11\% & 0.492 & +28\% & 0.424  & +18\%  & 9.115 & +298\% \\ %&--& --  \\
 
\bottomrule
\end{tabular}
\label{tab:boosting}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
% \end{wraptable}
%}

==> tables/tab_LPU_boosting_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
% \begin{wraptable}

%\begin{wraptable}[12]{r}{0.7\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{(Full Benchmark) Boosting effect of LPU layer for common deep learning backbones: MLP, LSTM, CNN and Attention.`+` indicates degraded performance.}\vspace{-1mm}
\scalebox{0.80}{
\begin{tabular}{c|c|cccccccccccccccccc}
%\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEL}&\multicolumn{2}{c|}{MLP}&\multicolumn{2}{c|}{LSTM}&\multicolumn{2}{c|}{lagged-LSTM}&\multicolumn{2}{c|}{CNN}&\multicolumn{2}{c}{Attention}\\
\midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\multicolumn{2}{c|}{Compare} & LPU  & Linear& LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030}  & +38\%   & 0.034  & +8.0\%  & 0.049 & +73\% & 0.093 & -21\% & 0.116   & -50\%   & 0.243  & -81\% \\
& 192  &\textbf{0.047} & +9.5\% & 0.049  & +30\%  & 0.174 & +32\% & 0.331 & -48\% & 0.101   & +20\%    & 0.387  & -86\% \\
& 336 & 0.063 & +5.8\% & \textbf{0.061}  & +64\%  & 0.119 & +84\% & 0.214 & -19\% & 0.122   & +25\%    & 1.652  & +12\% \\
& 720 &\textbf{0.081} & +1.4\%  & 0.082  & +62\%  & 0.184 & +32\% & 0.303 & -6.5\%  & 0.108   & +13\%    & 4.782  & -61\% \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.213}  & +136\%  & 0.431  & +121\%   & 0.291 & +56\% & 0.739 & -33\% & 0.310  & +43\%  & 0.805 & +23\% \\%&--& --
& 192 &\textbf{0.268} & +32\%   & 0.291 & +239\%   & 0.353  & +17\% & 0.535 & +15\% & 0.380  & +12\%  & 0.938 & +14\% \\%&--& --  \\
& 336 & 0.307& +0.1\%  & \textbf{0.296} & +235\%   & 0.436  & -6.7\% & 0.517 & +23\% & 0.359  & +29\% & 2.043 & -54\% & \\%&--& -- \\
& 720 & \textbf{0.321}& +37\%   & 0.339 & +196\%   & 0.636  & -11\% & 0.492 & +28\% & 0.424  & +18\%  & 9.115 & +298\% \\ %&--& --  \\
               
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
& 96  & 0.130 & +7.5\% & \textbf{0.110} & -18\% & 0.224 & +6.0\% & 0.521 & -58\% & 0.244 & -18\% & 0.338 & +872\% \\
& 192 & \textbf{0.205} & +39\% & 0.257 & -36\% & 0.787 & -35\% & 1.742 & -66\% & 0.630 & +2.1\% & 0.930 & +278\% \\
& 336 & 0.467 & +9.2\% & \textbf{0.461} & -33\% & 0.964 & +24\% & 2.281 & -38\% & 3.231 & -85\% & 1.067 & +69\%\\
& 720 & \textbf{1.003} & +26\% & 1.981 & -61\% & 2.703 & -29\% & 1.457 & +34\% & 5.531 & +9.7\% & 0.631 & +1831\% \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  &\textbf{0.312} & +18\% & 0.376 & +277\% & 0.215 & +1.2\% & 0.216 & +10\% & 0.543 & -33\% & 0.429 & +210\% \\
& 192 & \textbf{0.141} & +9.6\% & 0.199 & +598\% & 0.177 & +19\% & 0.186 & +17\% & 0.451 & +9.0\% & 0.476 & +176\% \\
& 336 & \textbf{0.143} & +2.5\% & 0.195 & +613\% & 0.192 & +19\% & 0.190 & +11\% & 0.346 & +44\% & 0.377 & +260\% \\
& 720 & \textbf{0.215} & +30\% & 0.240 & +475\% & 0.234 & -1.7\% & 0.250 & +15\% & 0.348 &  +47\% & 0.773 & +171\%\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 
& 96 & 0.0073 & -38\% & 0.006  & -33\% & 0.006 & -23\% & 0.0070 & -17\% & \textbf{0.0022} & +167\% & 0.0065 &-11\%\\
& 192 & 0.0106 & -64\% & 0.007 & -14\% & 0.0074 & -11\% & \textbf{0.0063} & -19\% & 0.007 & -24\% & 0.0075 & -12\%\\
& 336 & 0.0079 & -37\% & 0.006 & +4.9\% & 0.0056 & +12\% & \textbf{0.0055} & +12\% & 0.0056 & +0.5\% & 0.222 & -69\% \\
& 720 &0.0063 & +0.4\% & 0.006 & +7.6\% & \textbf{0.0062} & +5.3\% & 0.103 & -36\% &0.006 & +4.2\% & 0.037 & -81\% \\
                        
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & 1.393 &	+6.1\% & \textbf{1.220} & +36\% & 2.306 & +66\% & 4.189 & -9.2\% & 2.264 & -22\% & 2.249 & +217\% \\
& 36 & 1.242 & -22\% & \textbf{1.185} & +56\% & 2.950 & +44\% & 2.516 & +42\% & 1.841 & -3.0\% & 5.026 & +45\% \\
& 48 & 1.448 & -28\% & \textbf{1.079} & +79\% & 3.385 & +38\% & 3.501 & +16\% & 1.654 & +23\% & 2.838 & +115\% \\
& 60 & 2.089 & -18\% & \textbf{0.986} & +96\%  & 4.031 & +18\% & 4.258 & +10\% & 1.290 & +176\% & 4.978 & +250\% \\
\bottomrule
\end{tabular}
\label{tab:boosting}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}


==> tables/tab_ablation_FEL.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[ht]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.029} &\textbf{0.127}  &+0.0\%   & +0.0\%   & +12.1\% & +7.1\%    & +13.5\%   & +9.5\%   & +1.7\%  & +1.6\% &-- & -- \\
& 192  &\textbf{0.041} &\textbf{0.153}  &-1.5\% & -0.6\%  & +12.2\% & +8.5\%  & +10.8\%   & +7.8\%    & +2.0\%  & +3.3\% &-- & -- \\
& 336 & \textbf{0.053} & \textbf{0.175} &-1.7\% & -1.7\%  & +4.5\% & +4.0\%    & +10.8\%    & +6.3\%    & +4.5\% & +2.9\% &-- & --  \\
& 720 &\textbf{0.071}& \textbf{0.205}   &-0.9\%  & -1.0\%  & +5.5\% & +3.4\%  & +8.6\%    & +4.9\%    & +13.8\% & +7.8\% &-- & --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.154}  &\textbf{0.247}  &+155\%  & +81\%   & +160\% & +84\%    & +330\%  & +155\%  & +242\% & +119\% & 128\% & 83\% \\%&--& -- & \\
& 192 &\textbf{0.166} & \textbf{0.258} &+59\% & +39\%   & +121\%  & +67\%   & +224\%  & +117\%  & +264\% & +131\% & 124\% & 76\% \\%&--& --  \\
& 336 & \textbf{0.188}& \textbf{0.283} &+55\%  & +35\%   & +150\%  & +74\%   & +128\%  & +71\% & +183\% & +95\% & 117\% & 69\% \\%&--& -- \\
& 720 & \textbf{0.249}&\textbf{0.341}  &+33\%  & +25\%   & +154\%  & +73\%   & +192\%  & +95\%  & +312\% & +138\% & 89\% & 51\% \\ %&--& --  \\
                        
\bottomrule
\end{tabular}
\label{tab:ablation_FEL}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_FEL_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[!h]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{: (Full Benchmark)Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer.The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.8}{
\begin{tabular}{c|c|ccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& \\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.029} &\textbf{0.127}  &+0.0\%   & +0.0\%   & +12.1\% & +7.1\%    & +13.5\%   & +9.5\%   & +1.7\%  & +1.6\%  \\
& 192  &\textbf{0.041} &\textbf{0.153}  &-1.5\% & -0.6\%  & +12.2\% & +8.5\%  & +10.8\%   & +7.8\%    & +2.0\%  & +3.3\%  \\
& 336 & \textbf{0.053} & \textbf{0.175} &-1.7\% & -1.7\%  & +4.5\% & +4.0\%    & +10.8\%    & +6.3\%    & +4.5\% & +2.9\%   \\
& 720 &\textbf{0.071}& \textbf{0.205}   &-0.9\%  & -1.0\%  & +5.5\% & +3.4\%  & +8.6\%    & +4.9\%    & +13.8\% & +7.8\%   \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.154}  &\textbf{0.247}  &+155\%  & +81\%   & +160\% & +84\%    & +330\%  & +155\%  & +242\% & +119\%  \\%&--& -- & \\
& 192 &\textbf{0.166} & \textbf{0.258} &+59\% & +39\%   & +121\%  & +67\%   & +224\%  & +117\%  & +264\% & +131\%  \\%&--& --  \\
& 336 & \textbf{0.188}& \textbf{0.283} &+55\%  & +35\%   & +150\%  & +74\%   & +128\%  & +71\% & +183\% & +95\%  \\%&--& -- \\
& 720 & \textbf{0.249}&\textbf{0.341}  &+33\%  & +25\%   & +154\%  & +73\%   & +192\%  & +95\%  & +312\% & +138\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Exchange}} 

&96  &\textbf{0.110}  &\textbf{0.247}  &-13\%  & -12\%   & +51\% & +17\%    & +4.6\%  & -1.2\%  & -4.6\% & -5.8\%  \\%&--& -- & \\
& 192 &\textbf{0.207} & \textbf{0.352} &+7.2\% & +0.0\%   & +69\%  & +32\%   & +29\%  & +12\%  & +22\% & +11\%  \\%&--& --  \\
& 336 & \textbf{0.327}& \textbf{0.461} &+48\%  & +13\%   & +62\%  & +20\%   & +68\%  & +24\% & +72\% & +23\%  \\%&--& -- \\
& 720 & \textbf{0.811}&\textbf{0.708}  &+29\%  & +14\%   & +24\%  & +9.6\%   & +38\%  & +12\%  & +64\% & +27\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 

&96  &\textbf{0.144}  &\textbf{0.215}  &+69\%  & +47\%   & +13\% & +15\%    & +300\%  & +176\%  & +271\% & +161\%  \\%&--& -- & \\
& 192 &\textbf{0.120} & \textbf{0.199} &+17\% & +7.5\%   & +31\%  & +24\%   & +258\%  & +149\%  & +1572\% & +355\%  \\%&--& --  \\
& 336 & \textbf{0.128}& \textbf{0.212} &+6.2\%  & +7.6\%   & +16\%  & +15\%   & +151\%  & +102\% & +1514\% & +368\%  \\%&--& -- \\
& 720 & \textbf{0.153}&\textbf{0.252}  &+38\%  & +28\%   & +11\%  & +7.9\%   & +250\%  & +126\%  & +1048\% & +349\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 

&96  &\textbf{0.0012}  &\textbf{0.026}  &+17\%  & +6.2\%   & +16\% & +6.9\%    & +19\%  & +8.1\%  & +21\% & +8.9\%  \\%&--& -- & \\
& 192 &\textbf{0.0014} & \textbf{0.029} &-1.4\% & -2.4\%   & +5.0\%  & +1.7\%   & 0.7\%  & -0.7\%  & +4.3\% & +1.4\%  \\%&--& --  \\
& 336 & \textbf{0.0015}& \textbf{0.030} &+0.0\%  & -0.6\%   & +3.3\%  & +1.3\%   & +2.0\%  & +0.0\% & +3.3\% & +1.3\%  \\%&--& -- \\
& 720 & \textbf{0.0022}&\textbf{0.037}  &+4.6\%  & -0.3\%   & +4.1\%  & -1.6\%   & 3.6\%  & 0.0\%  & +0.0\% & -3.8\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{ILI}} 

&96  &\textbf{0.629}  &\textbf{0.538}  &+51\%  & +45\%   & -2.5\% & 9.5\%    & +20\%  & +29\%  & +112\% & +59\%  \\%&--& -- & \\
& 192 &\textbf{0.444} & \textbf{0.481} &+99\% & +58\%   & +25\%  & +24\%   & +84\%  & +56\%  & +360\% & +142\%  \\%&--& --  \\
& 336 & \textbf{0.557}& \textbf{0.584} &+33\%  & +31\%   & +21\%  & +16\%   & +58\%  & +30\% & +702\% & +94\%  \\%&--& -- \\
& 720 & \textbf{0.641}&\textbf{0.644}  &+8.4\%  & +5.4\%   & +23\%  & +18\%   & +42\%  & +22\%  & +74\% & +34\%  \\ %&--& --  \\
\bottomrule
\end{tabular}
\label{tab:ablation_FEL_full}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_FNO.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[ht]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030} &\textbf{0.128}  &+14\%   & +6.6\%   & +62\% & +31\%    & +286\%   & +118\%   & +709\%  & +166\% &-- & -- \\
& 192  &\textbf{0.047} &\textbf{0.160}  &+3.8\% & +2.2\%  & +271\% & +122\%  & +116\%   & +58\%    & +727\%  & +136\% &-- & -- \\
& 336 & \textbf{0.063} & \textbf{0.185} &-3.7\% & -2.1\%  & +90\% & +51\%    & +94\%    & +48\%    & +2524\% & +286\% &-- & --  \\
& 720 &\textbf{0.081}& \textbf{0.215}   &+0.9\%  & -0.6\%  & +127\% & +65\%  & +33\%    & +17\%    & +5783\% & +299\% &-- & --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
% &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

&96  &\textbf{0.213}  &\textbf{0.328}  &+103\%  & +40\%   & +37\% & +20\%    & +46\%  & +23\%  & +278\% & +105\% & 65\% & 38\% \\%&--& -- & \\
& 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & +249\% & +81\% & 39\% & 22\% \\%&--& --  \\
& 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & +564\% & +90\% & 33\% & 15\% \\%&--& -- \\
& 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +2739\% & +117\% & 47\% & 22\% \\ %&--& --  \\
                        
                        
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & \textbf{0.079} & \textbf{0.204} &0.139 &0.276 &0.197  &0.323 &1.292 &0.849 &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
%                         & 192 & \textbf{0.159} & \textbf{0.292} &0.256 &0.369 &0.300  &0.369 &1.631 &0.968 &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
%                         & 336 & \textbf{0.270} & \textbf{0.398} &0.426 &0.464 &0.509  &0.524 &2.225 &1.145 &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
%                         & 720 & \textbf{0.830} & \textbf{0.721} &1.090 &0.800 &1.447  &0.941 &2.521 &1.245 &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &\textbf{0.453}& \textbf{0.305} &0.562 &0.349 &0.613  &0.388 &0.824 &0.514 &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
%                         & 192 & \textbf{0.463} & \textbf{0.308} &0.562 &0.346 &0.616&0.382 &1.106 &0.672 &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
%                         & 336 & \textbf{0.483} & \textbf{0.321} &0.570 &0.323 &0.622  &0.337 &1.084 &0.627 &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
%                         & 720 & \textbf{0.562} & 0.383 &0.596 &\textbf{0.368} &0.660  &0.408 &1.536 &0.845 &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.199} & \textbf{0.262} &0.217  &0.296  &0.266  &0.336 &0.406 &0.444 &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
%                         & 192 & \textbf{0.228} & \textbf{0.288} &0.276  &0.336  &0.307  &0.367 &0.525 &0.527 &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
%                         & 336 &\textbf{0.267} &\textbf{0.323} & 0.339  &0.380  &0.359  &0.395 &0.531 &0.539 &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
%                         & 720 &\textbf{0.319} & \textbf{0.361} &0.403  &0.428 &0.578 &0.578 &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & \textbf{1.970} & \textbf{0.875} &2.203  &0.963  &3.483 &1.287 &4.631 &1.484 &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
%                         & 36 & \textbf{1.982} & \textbf{0.859} &2.272  &0.976  &3.103  &1.148 &4.123 &1.348 &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
%                         & 48 & \textbf{1.868} & \textbf{0.896} &2.209  &0.981  &2.669  &1.085 &4.066 &1.36 &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
%                         & 60 & \textbf{2.057} & \textbf{0.929} &2.545  &1.061  &2.770  &1.125 &4.278 &1.41 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:ablation_FNO}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_HiPPO.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of LPU layer. The original LPU block (whose projection and reconstruction matrix are fixed) is replaced with 6 variants (\textbf{Fixed} means the matrix are not trainable. \textbf{Trainable} means the matrix is initialized with original parameters and trainable. \textbf{Random Init} means the matrix is initialized randomly and trainable). The experiments are performed on ETTm1 and Electricity with different input lengths. The metric of variants is presented in relative value (`+` indicates degraded performance, `-` indicates improved performance).}
\vspace{-1mm}
\resizebox{\columnwidth}{!}{
\scalebox{0.60}{

\begin{tabular}{c|c|cccccccccccccccccc}
\toprule

\multicolumn{2}{c|}{Index}&\multicolumn{2}{c|}{Original}&\multicolumn{2}{c|}{Variant 1}&\multicolumn{2}{c|}{Variant 2}&\multicolumn{2}{c|}{Variant 3}&\multicolumn{2}{c|}{Variant 4}&\multicolumn{1}{c|}{Variant 5}&\multicolumn{2}{c}{Variant 6}\\
\midrule

\multicolumn{2}{c|}{Projection}&\multicolumn{4}{c|}{Fixed}&\multicolumn{6}{c|}{Trainable}&\multicolumn{1}{c|}{Random Init}&\multicolumn{2}{c}{Linear}\\
\midrule
\multicolumn{2}{c|}{Reconstruction}&\multicolumn{2}{c|}{Fixed}&\multicolumn{2}{c|}{Trainable}&\multicolumn{2}{c|}{Fixed}&\multicolumn{2}{c|}{Trainable}&\multicolumn{2}{c|}{Random Init}&\multicolumn{1}{c|}{--}&\multicolumn{2}{c}{Linear}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& -- & MSE  & MAE \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
%                         & 192 & \textbf{0.240} & \textbf{0.313} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
%                         & 336 & \textbf{0.286} & \textbf{0.345} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
%                         & 720 & \textbf{0.393} & \textbf{0.410} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
% \midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030} &\textbf{0.128}    &+6.0\%  & +3.1\% & +4.6\% & +3.1\%  & +4.7\%   & +2.7\%   & +0.7\% & +0.6\%  & NaN & +38\% & +22\%  \\
& 192  &\textbf{0.047} &\textbf{0.160}  &-2.6\%  & -1.3\%    & +2.5\% & +1.8\%  & -0.4\%   & +0.4\%   & -3.0\% & -1.0\%  & NaN  & +9.5\%  & +8.7\% \\
& 336 & \textbf{0.063} & \textbf{0.185} &+4.2\% & +1.8\%    & -2.4\% & -0.4\%  & -6.3\%   & -2.5\%    & +2.2\% & +1.4\%   & NaN & +5.8\% & +5.0\% \\
& 720 &\textbf{0.081}& \textbf{0.215}   &-0.4\%     & -0.6\%     &+24\%    & +12\%  & +11\%    & +5.9\%   & NaN & NaN       & NaN      & +1.4\%  & +2.2\% \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Electricity}}
&96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% & +11\% & +4.8\%  &NaN & +136\% & +58\%  \\
& 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &NaN  & +32\%  & +16\% \\
& 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &NaN & +0.1\% & -5.0\% \\
& 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &NaN  & 37\%  & 22\% \\

\bottomrule
\end{tabular}
\label{tab:ablation_HiPPO}
}}
% \end{adjustwidth}
%\end{footnotesize}
\vskip -0.05in
\end{table*}

%}

==> tables/tab_ablation_normalize.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\vskip -0.15in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of Normalization and Multiscale. Multiscale use 3 branches with: $T$, $2T$, and $4T$ as input sequence length. T is the predicted sequence length}\vspace{-1mm}
\scalebox{0.7}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c|}{ETTm2}&\multicolumn{2}{c|}{Electricity}&\multicolumn{2}{c|}{Exchange}&\multicolumn{2}{c|}{Traffic}&\multicolumn{2}{c|}{Weather}&\multicolumn{2}{c}{Illness}&\multicolumn{2}{c}{}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & Relative & MSE & Relative & MSE & Relative & MSE & Relative & MSE & Relative & MSE & Relative &\\
\midrule


\multirow{4}{*}{\rotatebox{90}{Methods}} 

&Original  &0.301 & +16\% & 0.195 & +4.8\% & 0.534 & + 60\% & 0.528 & +19\% & 0.264 & +4.9\% & 3.55 & + 80\% \\

& Normalization & 0.268 & +3.6\% & 0.199 & +6.4\% & 0.456 & +36\% & 0.656 & +48\% & 0.256 & +1.5\% & 3.36 & +70\% \\	
% &\textbf{0.047} &\textbf{0.160}  &-12\%  & -10\% & +2.5\% & +1.8\% & -0.4\%    & +0.4\%   & -\% & -\%  &--& --  \% \\
& Multiscale & 0.259 & + 0.19\% &	0.187 &   +0\%	& 0.335	 & 0\% & 0.541 & +22\% & 0.253 & +0.50\% &	2.41 & +22\% \\
& With both & 0.271	& +4.7\% &	0.189	& +1.5\% & 0.398 & +19\% & 0.442 & +0\% &  0.253 & +0.4\% & 1.97 & +0\% \\
% & 720 &\textbf{0.081}& \textbf{0.215}   &-0.\%     & -0.\%    & +\%    &  +\%   & +11\%    & +5.9\%   & -- & --       &--& - \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
% % &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% % & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% % & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% % & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

% &96  &\textbf{0.213}  &\textbf{0.328}  &+100\%  & +100\%   & +37\% & +20\%    & +46\%  & +23\%  & +11\% & +4.8\%  \\%&--& -- & \\
% & 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & -5.3\% & -3.9\%  \\%&--& --  \\
% & 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & -8.5\% & -9.0\% \\%&--& -- \\
% & 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +207\% & +85\% \\ %&--& --  \\
                        

\bottomrule
\end{tabular}
\label{tab:ablation_normalize}
}
\vskip -0.05in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/tab_ett_m.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Multivariate long-term forecasting results on ETT full benchmark. The best results are highlighted in bold. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
& 96 &\textbf{0.371} &\textbf{0.394} &0.376 &0.419  & 0.449& 0.459 &0.949 &0.777 & 0.865 & 0.713& 0.878& 0.740& 0.837& 0.728\\
& 192 &\textbf{0.414} &\textbf{0.423} &0.420 &0.448  & 0.500& 0.482 &0.882 &0.745 & 1.008 & 0.792& 1.037& 0.824& 0.923& 0.766\\
& 336 &\textbf{0.442} &\textbf{0.445} &0.459 &0.465  & 0.521& 0.496 &0.965 &0.75 & 1.107 & 0.809& 1.238& 0.932& 1.097& 0.835\\
& 720 &\textbf{0.465} &\textbf{0.472} &0.506 &0.507  & 0.514& 0.512 &1.074&0.814 & 1.181 &0.865&  1.135& 0.852& 1.257& 0.889\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
& 96  &\textbf{0.284} &\textbf{0.348} &0.346 &0.388 & 0.358& 0.397 &1.551&	0.968 & 3.755& 1.525& 2.116& 1.197 &2.626 &1.317\\
& 192 &\textbf{0.357} &\textbf{0.400} &0.429 &0.439 & 0.456& 0.452 &2.336	 &1.229 & 5.602& 1.931& 4.315& 1.635 &11.12 &2.979\\
& 336 &\textbf{0.377} &\textbf{0.417} &0.482 &0.480 & 0.482& 0.486 &2.801	 &1.259 & 4.721& 1.835& 1.124& 1.604 &9.323 &2.769\\
& 720 &\textbf{0.439} &\textbf{0.456} & 0.463 & 0.474 & 0.515& 0.511 &2.973	 &1.333 & 3.647& 1.625& 3.188& 1.540 &3.874 &1.697\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
& 96  &\textbf{0.302} &\textbf{0.345} &0.378 &0.418 & 0.505& 0.475 &0.640	 &0.584 & 0.672& 0.571& 0.600& 0.546 &0.538 &0.528\\
& 192 &\textbf{0.338} &\textbf{0.368} & 0.426 & 0.441 & 0.553& 0.496 &0.570	 &0.555 & 0.795& 0.669& 0.837& 0.700 &0.658 &0.592\\
& 336 &\textbf{0.373} &\textbf{0.388} & 0.445 & 0.459 & 0.621& 0.537 &0.795& 0.691& 1.212& 0.871& 1.124& 0.832 &0.898 &0.721\\
& 720 &\textbf{0.420} &\textbf{0.420} & 0.543 & 0.490 & 0.671& 0.561 &0.738 &0.655 & 1.166& 0.823& 1.153& 0.820 &1.102 &0.841\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 &\textbf{0.165} &\textbf{0.256} & 0.203 & 0.287 &0.255  &0.339  &0.705	 &0.690  &0.365  &0.453  &0.768  &0.642  &0.658  &0.619 \\
                        & 192 &\textbf{0.222} &\textbf{0.296} & 0.269 & 0.328 &0.281 &0.340  &0.924	 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827 \\
                        & 336 &\textbf{0.277} &\textbf{0.333} & 0.325 & 0.366  &0.339  &0.372  &1.364	 & 0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972 \\
                        & 720 &\textbf{0.371} &\textbf{0.389} & 0.421 & 0.415  &0.422  &0.419  &2.074 &1.074  &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242 \\
\bottomrule
\end{tabular}
}
\label{tab:multi-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
% \vskip -0.1in
\end{table*}



==> tables/tab_ett_u.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term forecasting results on ETT full benchmark. The best results are highlighted in bold. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
&96 &\textbf{0.055}&\textbf{0.178}&0.079 &0.215 &0.071 &0.206 &0.316 &0.490 &	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
&192 &\textbf{0.072}&\textbf{0.207}&0.104 &0.245 & 0.114&	0.262 & 0.345&0.516 &	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
&336 &\textbf{0.083}&\textbf{0.229}&0.119 &0.270 &0.107&0.258 &0.825 &0.846 &	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
&720 &\textbf{0.090}&\textbf{0.240}&0.127 &0.280 &0.126&0.283 &0.190 &0.355 &	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
&96 &\textbf{0.127}&0.272&0.128 &\textbf{0.271} & 0.153&	0.306 & 0.381&0.501 &	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
&192 &\textbf{0.182}&0.335&0.185 &\textbf{0.330} & 0.204&	0.351 & 0.332&0.458 &	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
&336 &\textbf{0.204}&\textbf{0.367}&0.231 &0.378 & 0.246&	0.389 & 0.655&0.670 &	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
&720 &\textbf{0.241}&\textbf{0.396}&0.278 &0.420 & 0.268&	0.409 & 0.630&0.662 &	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
&96 &\textbf{0.029}&\textbf{0.127}&0.033 &0.140 & 0.056&	0.183 & 0.651&0.733 &	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
&192 &\textbf{0.041}&\textbf{0.153}&0.058 &0.186 & 0.081&	0.216 & 0.190& 0.372&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
&336 &\textbf{0.053}&\textbf{0.175}&0.071 &0.209 & 0.076&	0.218 & 0.428&0.581 &	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
&720 &\textbf{0.071}&\textbf{0.205}&0.102 &0.250 & 0.110&	0.267 & 0.254&0.433 &	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 &0.065&\textbf{0.189}&\textbf{0.063} &0.189 & 0.065 & 0.189  & 0.153&0.318 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 &\textbf{0.094}&\textbf{0.233}& 0.102 & 0.245 & 0.118 & 0.256  &0.183 &0.350 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 &\textbf{0.124}&\textbf{0.274}& 0.130 & 0.279 & 0.154 & 0.305  &0.204 &0.367  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 &\textbf{0.173}&\textbf{0.323}& 0.178 & 0.325 & 0.182 &0.335  &0.482 &0.567  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
\end{table*}

==> tables/tab_low_ran_approximation_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

%\begin{wraptable}[9]{r}{0.6\textwidth}
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) univariate forecasting study for frequency enhanced layer: Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 

&96&0.065&0.189&0.064&0.185&\textbf{0.064}&\textbf{0.185}&0.064&0.186 \\

&192&0.094&0.233&0.094&0.231&0.093&0.231&\textbf{0.093}&\textbf{0.231} \\

&336&0.124&0.274&0.124&0.270&\textbf{0.124}&\textbf{0.269}&0.124&0.271 \\

&720&0.173&0.323&0.173&0.322&\textbf{0.173}&\textbf{0.322}&0.177&0.328 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 

&96&\textbf{0.154}&\textbf{0.247}&0.211&0.324&0.216&0.331&0.277&0.387 \\

&192&\textbf{0.166}&\textbf{0.258}&0.251&0.352&0.246&0.347&0.334&0.421 \\

&336&\textbf{0.188}&\textbf{0.283}&0.276&0.369&0.302&0.396&0.363&0.440 \\

&720&\textbf{0.249}&\textbf{0.341}&0.336&0.429&0.342&0.436&0.411&0.481 \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

&96&0.110&0.259&0.119&0.273&\textbf{0.104}&\textbf{0.247}&0.105&0.251 \\

&192&0.207&0.352&0.196&0.355&\textbf{0.195}&\textbf{0.349}&0.212&0.372 \\

&336&\textbf{0.327}&\textbf{0.461}&0.388&0.497&0.373&0.491&0.407&0.506 \\

&720&\textbf{0.811}&\textbf{0.708}&0.908&0.767&1.288&0.941&1.840&1.153 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 

&96&\textbf{0.144}&\textbf{0.215}&0.146&0.223&0.154&0.237&0.267&0.373 \\

&192&\textbf{0.120}&\textbf{0.199}&0.121&0.201&0.138&0.231&0.218&0.333 \\

&336&0.128&0.212&\textbf{0.120}&\textbf{0.206}&0.132&0.227&0.216&0.335 \\

&720&\textbf{0.153}&\textbf{0.252}&0.155&0.257&0.154&0.257&0.246&0.366 \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 

&96&0.0012&0.026&0.0011&0.025&\textbf{0.001}&\textbf{0.025}&0.001&0.025 \\

&192&0.0014&0.029&0.0014&0.028&\textbf{0.001}&\textbf{0.028}&0.001&0.028 \\

&336&0.0015&0.03&0.0015&0.030&\textbf{0.001}&\textbf{0.029}&0.002&0.030 \\

&720&0.0022&0.037&0.0022&0.037&\textbf{0.002}&\textbf{0.037}&0.002&0.037 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ILI$}} 

&96&0.629&0.538&\textbf{0.599}&\textbf{0.556}&0.628&0.558&0.630&0.579 \\

&192&\textbf{0.444}&\textbf{0.481}&0.487&0.533&0.508&0.561&0.570&0.612 \\

&336&0.557&0.584&\textbf{0.553}&\textbf{0.565}&0.703&0.696&0.722&0.706 \\

&720&\textbf{0.641}&\textbf{0.644}&0.648&0.641&0.900&0.780&1.493&1.032 \\

\midrule
\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{6.4\%}&\multicolumn{2}{c|}{1.6\%}&\multicolumn{2}{c}{0.4\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA_FULL}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}

==> tables/tab_low_rank_approximation.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

%\begin{wraptable}[9]{r}{0.6\textwidth}
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) study for frequency enhanced layer: Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}} 

&96  &\textbf{0.371} &\textbf{0.394}    &0.371  &0.397  &0.373  &0.399   & 0.391   & 0.418    \\
& 192  &0.414 &\textbf{0.423}  &0.414  &0.425  &\textbf{0.413}  &0.426   &  0.437  &  0.445    \\
& 336 & \textbf{0.442} & 0.445 &0.452  &0.451  &0.445  &\textbf{0.444}   &0.460    &0.458       \\
& 720 &\textbf{0.454}& \textbf{0.451}   &0.460  &0.472  &0.461  &0.471   &0.464    &0.476      \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 

&96  &\textbf{0.199} &\textbf{0.262}    &0.200  &0.266  &0.199  &0.263   &0.198    &0.261      \\
& 192  &0.228 &0.288  &0.232  &0.298  &0.227  &0.287   &\textbf{0.226}    &\textbf{0.285}       \\
& 336 & 0.267 & 0.323 &0.266  &0.320  &\textbf{0.253}  &\textbf{0.314}   &0.264    &0.316       \\
& 720 &0.319& 0.361   &\textbf{0.314}  &\textbf{0.352}  &0.319  &0.361   &0.314    &0.354      \\

\midrule
\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{6.4\%}&\multicolumn{2}{c|}{1.6\%}&\multicolumn{2}{c}{0.4\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}

==> tables/tab_lra_3d.tex <==
%\resizebox{!}{\.5\paperheight}{

% \begin{wraptable}[11]{r}{0.6\textwidth}
\vskip -0.15in
% \begin{wraptable}{r}{0.6\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) study for Frequency Enhanced Layer (FEL): Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}\vspace{-1.5mm}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{ETTh1}} 

&96  &\textbf{0.371} &\textbf{0.394}    &0.371  &0.396  &0.371  &0.398   & 0.400   & 0.421    \\
& 192  &0.414 &\textbf{0.423}  &0.411  &0.423  &0.414  &0.426   & 0.435   & 0.444    \\
& 336 & \textbf{0.442} & 0.445 &0.443  &0.446  &0.443  & 0.444  & 0.492   &  0.478     \\
& 720 &\textbf{0.454}& \textbf{0.451}   &0.464  &0.474  &0.468  &0.478   & 0.501   & 0.499      \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Weather}} 
&96  &\textbf{0.199} &\textbf{0.262}   &0.199  &0.263  &0.197  &0.262   &0.198    & 0.263     \\
& 192  &0.228 &0.288  &0.225  &0.285  &0.226  &0.285   &0.225    & 0.286      \\
& 336 & 0.267 & 0.323 &0.266  &0.321  &0.263  &0.314   & 0.264   &  0.316      \\
& 720 &0.319& 0.361  &0.314 &0.355  &0.315  & 0.354   &0.318    & 0.357   \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.079  &0.202  &0.081  &0.206   &0.084    &0.211     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.152  &0.287  &0.163  &0.299   &0.176    &0.313     \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.301  &0.411  &0.340  &0.439   &0.368    &0.459      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &0.952  &0.726  &1.229  &0.833   &1.705    &1.021     \\
% \midrule

\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{1.95\%}&\multicolumn{2}{c|}{0.41\%}&\multicolumn{2}{c}{0.10\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
% \end{wraptable}
%}

==> tables/tab_mean_std.tex <==
\vspace{-.2cm}
\begin{table}[ht]
%\setlength{\uppercaptionskip}{0.pt}
%\setlength{\belowcaptionskip}{-0.pt}
% \label{sample-table-kstest}
%\vskip 0.15in
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{MSE with error bars (Mean and STD) for FiLM and FEDformer baseline for multivariate long-term forecasting. All experiments are repeated 5 times.}
\begin{small}
% \begin{sc}
\scalebox{0.75}{
\begin{tabular}{c|c|ccccc}
\toprule
\multicolumn{2}{c|}{MSE}& ETTm2 & Electricity & Exchange & Traffic\\ %&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\midrule
\multirow{4}{*}{\rotatebox{90}{FiLM}} 
& 96 & 0.165 $\pm$ 0.0051 & 0.153$\pm$ 0.0014 & 0.079$\pm$ 0.002 & 0.416$\pm$ 0.010 \\
& 192 & 0.222 $\pm$ 0.0038 & 0.165$\pm$ 0.0023 & 0.159$\pm$ 0.011 & 0.408$\pm$ 0.007 \\
& 336 & 0.277 $\pm$ 0.0021 & 0.186$\pm$ 0.0018 & 0.270$\pm$ 0.018 & 0.425$\pm$ 0.007 \\
& 720 & 0.371 $\pm$ 0.0066 & 0.236$\pm$ 0.0022 & 0.536$\pm$ 0.026 & 0.520$\pm$ 0.003 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{FED-f}} 
& 96 & 0.203 $\pm$ 0.0042 & 0.194 $\pm$ 0.0008 & 0.148 $\pm$ 0.002 & 0.217 $\pm$ 0.008 \\
& 192 & 0.269 $\pm$ 0.0023 & 0.201$\pm$ 0.0015 & 0.270$\pm$ 0.008 & 0.604 $\pm$ 0.004 \\
& 336 & 0.325 $\pm$ 0.0015 & 0.215$\pm$ 0.0018 & 0.460$\pm$ 0.016 & 0.621 $\pm$ 0.006 \\
& 720 & 0.421 $\pm$ 0.0038 & 0.246$\pm$ 0.0020 & 1.195$\pm$ 0.026 & 0.626 $\pm$ 0.003 \\
\bottomrule
\end{tabular}
}
\label{tab:std}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}




==> tables/tab_mode_selection_policy.tex <==
% \begin{wraptable}[16]{r}{0.6\textwidth}
\begin{table*}[h]

% \begin{wraptable}[11]{r}{0.5\textwidth}
\vskip -0.1in

\centering
\caption{Mode selection policy study for frequency enhanced layer. Lowest: select the lowest $m$ frequency mode; Random: select $m$ random frequency mode; Low random: select the $0.8*m$ lowest frequency mode and $0.2*m$ random high frequency mode.}\vspace{-1.5mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Policy}&\multicolumn{2}{c|}{Lowest}&\multicolumn{2}{c|}{Random}&\multicolumn{2}{c}{Low random}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\
\midrule

\multirow{4}{*}{\rotatebox{90}{Exchange}} 

&96  &\textbf{0.086} &\textbf{0.204}    &0.086  &0.208  &0.087  &0.210        \\
& 192  &0.188 &\textbf{0.292}  &\textbf{0.187}  &0.318  &0.207  &0.340      \\
& 336 & 0.356 & \textbf{0.433} &0.358  &0.437  &\textbf{0.353}  &0.461   \\
& 720 &\textbf{0.727}& \textbf{0.669}   &0.788  &0.680  &0.748  &0.674   \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Weather}} 

&96  &0.199 &0.262 &0.197  &0.256  &\textbf{0.196}  &\textbf{0.254}   \\
& 192  &\textbf{0.228} &\textbf{0.288}  &0.234  &0.300  &0.234  &0.301   \\
& 336 & 0.267 & 0.323 &0.266  &0.319  &\textbf{0.263}  &\textbf{0.316}   \\
& 720 &0.319& 0.361 &0.317  &0.356  &\textbf{0.316}  &\textbf{0.354}  \\

\bottomrule

\end{tabular}
\label{tab:mode}
}
\end{table*}
% \end{wraptable}


==> tables/tab_mode_selection_policy_full.tex <==
% \begin{wraptable}[16]{r}{0.6\textwidth}
\begin{table*}[h]

% \begin{wraptable}[11]{r}{0.5\textwidth}
\vskip -0.1in

\centering
\caption{Mode selection policy study for frequency enhanced layer. Lowest: select the lowest $m$ frequency mode; Random: select $m$ random frequency mode; Low random: select the $0.8*m$ lowest frequency mode and $0.2*m$ random high frequency mode.}\vspace{-1.5mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Policy}&\multicolumn{2}{c|}{Lowest}&\multicolumn{2}{c|}{Random}&\multicolumn{2}{c}{Low random}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
&96&\textbf{0.065}&\textbf{0.189}&0.066&0.189&0.066&0.190 \\

&192&\textbf{0.094}&\textbf{0.233}&0.096&0.235&0.096&0.235 \\

&336&\textbf{0.124}&0.274&0.125&\textbf{0.270}&0.128&0.275 \\

&720&0.173&0.323&\textbf{0.173}&\textbf{0.322}&0.173&0.323 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
&96&\textbf{0.154}&\textbf{0.247}&0.175&0.0.260&0.176&0.262 \\

&192&\textbf{0.166}&\textbf{0.258}&0.177&0.266&0.168&0.273 \\

&336&\textbf{0.188}&\textbf{0.283}&0.199&0.289&0.192&0.299 \\

&720&\textbf{0.249}&\textbf{0.341}&0.269&0.364&0.270&0.362 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Exchange}} 
&96&0.11&0.259&0.110&0.256&\textbf{0.106}&\textbf{0.249} \\

&192&0.207&0.352&\textbf{0.196}&\textbf{0.351}&0.207&0.357 \\

&336&\textbf{0.327}&\textbf{0.461}&0.451&0.522&0.373&0.484 \\

&720&0.811&0.708&0.835&0.714&\textbf{0.604}&\textbf{0.628} \\


\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 
&96&\textbf{0.144}&\textbf{0.215}&0.145&0.216&0.145&0.217 \\

&192&0.12&0.199&0.119&0.198&\textbf{0.118}&\textbf{0.197} \\

&336&0.128&0.212&\textbf{0.122}&\textbf{0.207}&0.122&0.209 \\

&720&0.153&0.252&\textbf{0.142}&\textbf{0.238}&0.155&0.259 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
&96&\textbf{0.0012}&\textbf{0.026}&0.0012&0.027&0.0012&0.026 \\

&192&\textbf{0.0014}&\textbf{0.029}&0.0014&0.029&0.0014&0.029 \\

&336&\textbf{0.0015}&\textbf{0.03}&0.0015&0.030&0.0015&0.030 \\

&720&\textbf{0.0022}&\textbf{0.037}&0.0023&0.037&0.0023&0.037 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{ILI}} 
&96&0.629&0.538&0.639&0.542&\textbf{0.626}&\textbf{0.537} \\

&192&\textbf{0.444}&\textbf{0.481}&0.448&0.490&0.447&0.494 \\

&336&\textbf{0.557}&\textbf{0.584}&0.560&0.590&0.557&0.587 \\

&720&\textbf{0.641}&\textbf{0.644}&0.641&0.647&0.643&0.650 \\



\bottomrule

\end{tabular}
\label{tab:mode_full}
}
\end{table*}
% \end{wraptable}


==> tables/tab_noise_injection.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Noise injection studies. A 0.3*$\mathcal{N}\left(0,1\right)$ Gaussian noise is introduced into our training/testing. We conduct 4 sets of experiments with/without noise in training and test phases. The experiments are performed on ETTm1 and Electricity with different output lengths. The metric of variants is presented in relative value ('+' indicates degraded performance, and '-' indicates improved performance).}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule

\multicolumn{2}{c|}{Training}&\multicolumn{4}{c|}{noise}&\multicolumn{4}{c}{with noise}\\
\midrule
\multicolumn{2}{c|}{Testing}&\multicolumn{2}{c|}{without noise}&\multicolumn{2}{c|}{with noise}&\multicolumn{2}{c|}{without noise}&\multicolumn{2}{c}{with noise}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
%                         & 192 & \textbf{0.240} & \textbf{0.313} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
%                         & 336 & \textbf{0.286} & \textbf{0.345} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
%                         & 720 & \textbf{0.393} & \textbf{0.410} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
% \midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}} 

&96  &\textbf{0.371} &\textbf{0.394}    &-1.6\%  & -2.0\% & -0.0\% & -0.0\%  & -1.6\%   & -2.0\%     \\
& 192  &\textbf{0.414} &\textbf{0.423}  &-0.5\%  & -1.4\%    & +0.5\% & -0.0\%  & -0.5\%   & -1.4\%    \\
& 336 & \textbf{0.442} & \textbf{0.445} &-1.8\% & -0.9\%    & -0.9\% & +1.3\%  & -3.2\%   & -1.6\%     \\
& 720 &\textbf{0.465}& \textbf{0.472}   &+0.2\%     & -0.2\%     &+0.9\%    & +0.9\%  & -0.6\%    & -0.4\%    \\

% \midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:ablation_noise}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/tab_parameter_size.tex <==
\begin{table}[h]
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{Parameter size of baseline models and FiLM with different low-rank approximations: the models are trained and tested on ETT dataset; the subscript number denotes $k$ in low-rank approximation.}
\begin{small}
% \begin{sc}
\vskip 0.05in
\begin{tabular}{c|ccccccc}
\toprule
Methods&Transformer&Autoformer&FEDformer&FiLM&$\mathrm{FiLM}_{16}$ & $\mathrm{FiLM}_4$ & $\mathrm{FiLM}_1$\\
\midrule
Parameter(M) & 0.0069 & 0.0069& 0.0098& 1.50 & 0.0293 &0.0062& 0.00149 \\
%&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\bottomrule
\end{tabular}
\label{tab:size}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}


==> tables/tab_rebuttal_nhits.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h!]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). Supplementary results of non-Transformer baselines (N-Hits and a seasonal-naive model).}
% \vspace{-1mm}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccccccccc|}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{N-Hits}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Seasonal-naive}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
                        &96 & \textbf{0.165} & 0.256 & 0.176 & \textbf{0.255} &0.203 &0.287 &0.255  &0.339  &0.262 &0.300 \\
                        & 192 & \textbf{0.222} & \textbf{0.296} & 0.245 & 0.305 & 0.269  &0.328  &0.281 &0.340  &0.319 &0.337\\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.295 & 0.346 & 0.325 &0.366 &0.339  &0.372  &0.375 &0.371\\
                        & 720 & \textbf{0.371} & \textbf{0.389} & 0.401 & 0.426 & 0.421 &0.415 &0.422  &0.419 &0.469 &0.422\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
                        &96  &0.154  &0.267 & \textbf{0.147} & \textbf{0.249}  &0.183 &0.297 &0.201  &0.317 &0.211 &0.278\\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.167 & 0.269 & 0.195 &0.308 &0.222  &0.334 &0.214 &0.282\\
                        & 336 & 0.188 & \textbf{0.283} & \textbf{0.186} & 0.290 & 0.212 &0.313 &0.231 &0.338 &0.226 &0.294\\
                        & 720 & 0.236 & \textbf{0.332} & 0.243 & 0.340 &\textbf{0.231} &0.343 &0.254  &0.361 &0.265 & 0.324\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
                        &96  & \textbf{0.086} & \textbf{0.204} &0.092 & 0.211 & 0.139 & 0.276 & 0.197 &0.323 &0.086 &0.204 \\
                        & 192 & \textbf{0.189} & \textbf{0.292} & 0.208 & 0.322 &0.256 &0.369 & 0.300 & 0.369 &0.172 &0.295\\
                        & 336 & \textbf{0.356} & \textbf{0.433} & 0.371 & 0.443 & 0.426 &0.464 & 0.509 & 0.524 &0.311 &0.401\\
                        & 720 & \textbf{0.727} & \textbf{0.669} & 0.888 & 0.723 &  1.090 &0.800 & 1.447 & 0.941 &0.832 &0.686\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
                        &96  & 0.416& 0.294 & \textbf{0.402} & \textbf{0.282} & 0.562 &0.349 &0.613  &0.388 &1.219 &0.497\\
                        & 192 & \textbf{0.408} & \textbf{0.288} &0.420 & 0.297 & 0.562 &0.346 &0.616&0.382 &1.089 &0.456\\
                        & 336 & \textbf{0.425} & \textbf{0.298} &0.448 & 0.313 & 0.570 &0.323 &0.622  &0.337 &1.147 &0.473\\
                        & 720 & \textbf{0.520} &\textbf{0.353} &0.539 & 0.353 & 0.596 &0.368 &0.660  &0.408 &1.181 &0.486\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} 
                        & 96 & 0.199 & 0.262 & \textbf{0.158} & \textbf{0.195} & 0.217  &0.296  &0.266  &0.336 &0.315 &0.288\\
                        & 192 & 0.228 & 0.288 & \textbf{0.211} & \textbf{0.247} & 0.276  &0.336  &0.307  &0.367 &0.341 &0.305\\
                        & 336 &\textbf{0.267} & 0.323 & 0.274 & \textbf{0.300} & 0.339  &0.380  &0.359  &0.395 &0.381 &0.331\\
                        & 720 &\textbf{0.319} & 0.361 &0.351 & \textbf{0.353} & 0.403  &0.428 &0.578 &0.578 &0.440 &0.370 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
                        & 24 & 1.970 & 0.875 & \textbf{1.862} & \textbf{0.869} & 2.203  &0.963  &3.483 &1.287 &6.581 &1.699 \\
                        & 36 & \textbf{1.982} & \textbf{0.859} &2.071 & 0.969 & 2.272  &0.976  &3.103  &1.148 &7.121 &1.882 \\
                        & 48 & \textbf{1.868} & \textbf{0.896} &2.346 & 1.042 & 2.209  &0.981  &2.669  &1.085 &6.567 &1.797 \\
                        & 60 & \textbf{2.057} & \textbf{0.929} &2.560 & 1.073 & 2.545  &1.061  &2.770  &1.125 &5.885 &1.675 \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}


% %\resizebox{!}{\.5\paperheight}{
% % \vskip -0.2in
% \begin{table*}[h]
% \centering
% %\begin{footnotesize}
% % \begin{adjustwidth}{-1.5in}{-1in}
% \caption{Univariate Benchmark}
% % \vspace{-1mm}
% \scalebox{0.8}{
% \begin{tabular}{c|c|cccccccccccccc|}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{N-Hits}&\multicolumn{2}{c|}{N-BEATS}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
% & 96 & 0.065 & 0.189  & 0.066 & \textbf{0.185} & 0.082 & 0.219 &\textbf{0.063} &0.189 & 0.065 & 0.189 \\
% & 192& 0.094 & 0.233 & \textbf{0.087} & \textbf{0.223} & 0.120 & 0.268 &0.102 &0.245 & 0.118 & 0.256 \\
% & 336 & 0.124 & \textbf{0.274} & \textbf{0.106} &0.251&0.226 & 0.370& 0.130 &0.279 & 0.154 & 0.305  \\
% & 720 & \textbf{0.173} & 0.323 &0.178 &\textbf{0.312} &0.188 & 0.338 & 0.312&0.325 & 0.182 &0.335 \\
% \midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% &96  & 0.110 & 0.259 & \textbf{0.093} & \textbf{0.223} & 0.156 & 0.299 & 0.131 &0.284 & 0.241 & 0.387\\
% & 192 & \textbf{0.207} & 0.352& 0.230 & \textbf{0.313} &0.669  &0.665& 0.277 &0.420  &0.300  &0.369 \\
% & 336 & \textbf{0.327} & \textbf{0.461} &0.370 &0.486 &0.611 &0.605 &0.486&0.511 &0.509  &0.524 \\
% & 720 & 0.811 & 0.708 &\textbf{0.728} & \textbf{0.569}& 1.111 &0.860& 1.162 &0.832 &1.260  &0.867 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
% %                         &96  & 0.416& 0.294 & \textbf{0.402} & \textbf{0.282} & 0.562 &0.349 &0.613  &0.388 \\
% %                         & 192 & \textbf{0.408} & \textbf{0.288} &0.420 & 0.297 & 0.562 &0.346 &0.616&0.382\\
% %                         & 336 & \textbf{0.425} & \textbf{0.298} &0.448 & 0.313 & 0.570 &0.323 &0.622  &0.337\\
% %                         & 720 & \textbf{0.520} &\textbf{0.353} &0.539 & 0.353 & 0.596 &0.368 &0.660  &0.408 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$Weather$}} 
% %                         & 96 & 0.199 & 0.262 & \textbf{0.158} & \textbf{0.195} & 0.217  &0.296  &0.266  &0.336\\
% %                         & 192 & 0.228 & 0.288 & \textbf{0.211} & \textbf{0.247} & 0.276  &0.336  &0.307  &0.367\\
% %                         & 336 &\textbf{0.267} & 0.323 & 0.274 & \textbf{0.300} & 0.339  &0.380  &0.359  &0.395 \\
% %                         & 720 &\textbf{0.319} & 0.361 &0.351 & \textbf{0.353} & 0.403  &0.428 &0.578 &0.578 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$ILI$}} 
% %                         & 24 & 1.970 & 0.875 & \textbf{1.862} & \textbf{0.869} & 2.203  &0.963  &3.483 &1.287 \\
% %                         & 36 & \textbf{1.982} & \textbf{0.859} &2.071 & 0.969 & 2.272  &0.976  &3.103  &1.148 \\
% %                         & 48 & \textbf{1.868} & \textbf{0.896} &2.346 & 1.042 & 2.209  &0.981  &2.669  &1.085 \\
% %                         & 60 & \textbf{2.057} & \textbf{0.929} &2.560 & 1.073 & 2.545  &1.061  &2.770  &1.125 \\
% \bottomrule
% \end{tabular}
% \label{tab:multi-benchmarks}
% }
% % \end{adjustwidth}
% %\end{footnotesize}
% \end{table*}
%}

==> tables/tab_signal_recovery.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTm1$}} 

&96  &\textbf{0.030} &\textbf{0.128}  &+14\%   & +6.6\%   & +62\% & +31\%    & +286\%   & +118\%   & +709\%  & +166\% &-- & -- \\
% & 192  &\textbf{0.047} &\textbf{0.160}  &+3.8\% & +2.2\%  & +271\% & +122\%  & +116\%   & +58\%    & +727\%  & +136\% &-- & -- \\
% & 336 & \textbf{0.063} & \textbf{0.185} &-3.7\% & -2.1\%  & +90\% & +51\%    & +94\%    & +48\%    & +2524\% & +286\% &-- & --  \\
% & 720 &\textbf{0.081}& \textbf{0.215}   &+0.9\%  & -0.6\%  & +127\% & +65\%  & +33\%    & +17\%    & +5783\% & +299\% &-- & --  \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
% % &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% % & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% % & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% % & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

% &96  &\textbf{0.213}  &\textbf{0.328}  &+103\%  & +40\%   & +37\% & +20\%    & +46\%  & +23\%  & +278\% & +105\% & 65\% & 38\% \\%&--& -- & \\
% & 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & +249\% & +81\% & 39\% & 22\% \\%&--& --  \\
% & 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & +564\% & +90\% & 33\% & 15\% \\%&--& -- \\
% & 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +2739\% & +117\% & 47\% & 22\% \\ %&--& --  \\
                        
                        
\bottomrule
\end{tabular}
\label{tab:ablation_FNO}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/useless_tabs/tab_hyperparam.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long sequence time-series forecasting results on ETTm1, parameter sensitivity}
\vskip 0.05in
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
&96 &0.079 &0.215 &0.080 &0.214 &\textbf{0.071} &\textbf{0.206}&	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
&192 &\textbf{0.104} &\textbf{0.245} &0.105 &0.256 & 0.114&	0.262&	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
&336 &0.119 &0.270 &0.120 &0.269 &\textbf{0.107}&\textbf{0.258}&	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
&720 &0.142 &0.299 &0.127 &0.280 &\textbf{0.126}&\textbf{0.283}&	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
&96 &\textbf{0.128} &\textbf{0.271} &0.156 &0.306 & 0.153&	0.306&	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
&192 &\textbf{0.185} &\textbf{0.330} &0.238 &0.380 & 0.204&	0.351&	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
&336 &\textbf{0.231} &\textbf{0.378} &0.271 &0.412 & 0.246&	0.389&	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
&720 &0.278 &0.420 &0.288 &0.438 & \textbf{0.268}&	\textbf{0.409}&	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
&96 &\textbf{0.033} &\textbf{0.140} &0.036 &0.149 & 0.056&	0.183&	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
&192 &\textbf{0.058} &\textbf{0.186} &0.069 &0.206 & 0.081&	0.216&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
&336 &0.084 &0.231 &\textbf{0.071} &\textbf{0.209} & 0.076&	0.218&	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
&720 &\textbf{0.102} &0.250 &0.105 &\textbf{0.248} & 0.110&	0.267&	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.067 & 0.198 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
\end{table*}

% \begin{table*}[t]
% \centering
% % \begin{small}
% % \begin{adjustwidth}{-1.5in}{-1in}
% \caption{Univariate long sequence time-series forecasting results on ETT full benchmark. The best results are highlighted in bold.}
% \vskip 0.05in
% \scalebox{0.85}{
% \begin{tabular}{c|c|cccccccccccccccc}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
% \midrule

% \multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
% &96 &0.079 &0.215 &0.080 &0.214 &\textbf{0.071} &\textbf{0.206}&	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
% &192 &\textbf{0.104} &\textbf{0.245} &0.105 &0.256 & 0.114&	0.262&	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
% &336 &0.119 &0.270 &0.120 &0.269 &\textbf{0.107}&\textbf{0.258}&	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
% &720 &0.142 &0.299 &0.127 &0.280 &\textbf{0.126}&\textbf{0.283}&	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
% &96 &\textbf{0.128} &\textbf{0.271} &0.156 &0.306 & 0.153&	0.306&	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
% &192 &\textbf{0.185} &\textbf{0.330} &0.238 &0.380 & 0.204&	0.351&	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
% &336 &\textbf{0.231} &\textbf{0.378} &0.271 &0.412 & 0.246&	0.389&	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
% &720 &0.278 &0.420 &0.288 &0.438 & \textbf{0.268}&	\textbf{0.409}&	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
% &96 &\textbf{0.033} &\textbf{0.140} &0.036 &0.149 & 0.056&	0.183&	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
% &192 &\textbf{0.058} &\textbf{0.186} &0.069 &0.206 & 0.081&	0.216&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
% &336 &0.084 &0.231 &\textbf{0.071} &\textbf{0.209} & 0.076&	0.218&	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
% &720 &\textbf{0.102} &0.250 &0.105 &\textbf{0.248} & 0.110&	0.267&	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
% & 96 & 0.067 & 0.198 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
% & 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
% & 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
% & 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:uni-benchmarks-ett}
% % \end{adjustwidth}
% % \end{small}
% \end{table*}


==> tables_vq/few_shot_10.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 10\% data. We use prediction length $O \in {96, 192, 336, 720}$.A lower MSE indicates better performance, and the best results are highlighted in bold. ’-’ means that 10\% time series is not sufficient to constitute a training set.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|ccccccccccccccccccc}

\toprule
\multicolumn{2}{c|}{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c|}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE \\
\midrule
\multirow{5}{*}{\rotatebox{90}{ETTm1}} 
 & 96  & 0.333          & 0.365          & 0.41  & 0.419 & 0.39  & 0.404  & 0.352 & 0.392 & 0.578 & 0.518  & 0.774 & 0.614 & 1.162 & 0.785 & 1.555 & 0.910 & 1.442 & 0.847 \\
 & 192 & 0.370          & 0.388          & 0.437 & 0.434 & 0.429 & 0.423  & 0.382 & 0.412 & 0.617 & 0.546  & 0.754 & 0.592 & 1.172 & 0.793 & 1.883 & 1.033 & 1.444 & 0.862 \\
 & 336 & 0.413          & 0.416          & 0.476 & 0.454 & 0.469 & 0.439  & 0.419 & 0.434 & 0.998 & 0.775  & 0.869 & 0.677 & 1.227 & 0.908 & 2.095 & 1.110 & 1.45  & 0.866 \\
 & 720 & 0.476          & 0.452          & 0.681 & 0.556 & 0.569 & 0.498  & 0.49  & 0.477 & 0.693 & 0.579  & 0.81  & 0.63  & 1.207 & 0.797 & 2.389 & 1.167 & 1.366 & 0.85  \\
 & Avg & \textbf{0.398} & \textbf{0.405} & 0.501 & 0.466 & 0.464 & 0.441  & 0.411 & 0.429 & 0.722 & 0.605  & 0.802 & 0.628 & 1.192 & 0.821 & 1.981 & 1.055 & 1.426 & 0.856 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Electricity}} 
 & 96  & 0.145          & 0.243          & 0.14  & 0.238 & 0.139 & 0.237  & 0.15  & 0.253 & 0.231 & 0.323  & 0.261 & 0.348 & 1.259 & 0.919 & 0.649 & 0.584 & 0.993 & 0.784 \\
 & 192 & 0.162          & 0.259          & 0.16  & 0.255 & 0.156 & 0.252  & 0.164 & 0.264 & 0.261 & 0.356  & 0.338 & 0.406 & 1.16  & 0.873 & 0.667 & 0.594 & 0.938 & 0.753 \\
 & 336 & 0.188          & 0.284          & 0.18  & 0.276 & 0.175 & 0.27   & 0.181 & 0.282 & 0.36  & 0.445  & 0.41  & 0.474 & 1.157 & 0.872 & 0.711 & 0.620 & 0.925 & 0.745 \\
 & 720 & 0.245          & 0.325          & 0.241 & 0.323 & 0.233 & 0.317  & 0.223 & 0.321 & 0.53  & 0.585  & 0.715 & 0.685 & 1.203 & 0.898 & 0.833 & 0.690 & 1.004 & 0.79  \\
 & Avg & \textbf{0.185} & \textbf{0.278} & 0.18  & 0.273 & 0.176 & 0.269  & 0.18  & 0.28  & 0.346 & 0.427  & 0.431 & 0.478 & 1.195 & 0.891 & 0.715 & 0.622 & 0.965 & 0.768 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}}
 & 96  & 0.409          & 0.272          & 0.403 & 0.289 & 0.414 & 0.297  & 0.419 & 0.298 & 0.639 & 0.4    & 0.672 & 0.405 & 1.557 & 0.821 & 0.928 & 0.513 & 1.527 & 0.815 \\
 & 192 & 0.423          & 0.275          & 0.415 & 0.296 & 0.426 & 0.301  & 0.434 & 0.305 & 0.637 & 0.416  & 0.727 & 0.424 & 1.454 & 0.765 & 0.976 & 0.530 & 1.538 & 0.817 \\
 & 336 & 0.428          & 0.279          & 0.426 & 0.304 & 0.434 & 0.303  & 0.449 & 0.313 & 0.655 & 0.427  & 0.749 & 0.454 & 1.521 & 0.812 & 1.015 & 0.545 & 1.55  & 0.819 \\
 & 720 & 0.445          & 0.296          & 0.474 & 0.331 & 0.487 & 0.337  & 0.484 & 0.336 & 0.722 & 0.456  & 0.847 & 0.499 & 1.605 & 0.846 & 1.162 & 0.607 & 1.588 & 0.833 \\
 & Avg & \textbf{0.426} & \textbf{0.281} & 0.430 & 0.305 & 0.44  & 0.31   & 0.447 & 0.313 & 0.663 & 0.425  & 0.749 & 0.446 & 1.534 & 0.811 & 1.020 & 0.549 & 1.551 & 0.821 \\

 
 
\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}} 
& 96  & 0.152          & 0.196          & 0.165 & 0.215 & 0.163 & 0.215  & 0.171 & 0.224 & 0.188 & 0.253  & 0.221 & 0.297 & 0.374 & 0.401 & 0.305 & 0.371 & 0.335 & 0.38  \\
 & 192 & 0.201          & 0.241          & 0.21  & 0.257 & 0.21  & 0.254  & 0.215 & 0.263 & 0.25  & 0.304  & 0.27  & 0.322 & 0.552 & 0.478 & 0.425 & 0.432 & 0.522 & 0.462 \\
 & 336 & 0.252          & 0.282          & 0.259 & 0.297 & 0.256 & 0.292  & 0.258 & 0.299 & 0.312 & 0.346  & 0.32  & 0.351 & 0.724 & 0.541 & 0.605 & 0.500 & 0.715 & 0.535 \\
 & 720 & 0.325          & 0.335          & 0.332 & 0.346 & 0.321 & 0.339  & 0.32  & 0.346 & 0.387 & 0.393  & 0.39  & 0.396 & 0.739 & 0.558 & 0.714 & 0.536 & 0.611 & 0.5   \\
 & Avg & \textbf{0.233} & \textbf{0.264} & 0.242 & 0.279 & 0.238 & 0.275  & 0.241 & 0.283 & 0.284 & 0.324  & 0.3   & 0.342 & 0.597 & 0.495 & 0.512 & 0.460 & 0.546 & 0.469 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Wind}}  
 & 96  & 0.907          & 0.627          & 1.070 & 0.717 & 1.075 & 0.718  & 1.012 & 0.697 & 1.490 & 0.911  & 1.464 & 0.905 & 5.424 & 1.935 & 3.858 & 1.649 & 2.570 & 1.331 \\
 & 192 & 1.150          & 0.757          & 1.331 & 0.836 & 1.342 & 0.843  & 1.266 & 0.820 & 1.671 & 0.977  & 1.850 & 1.047 & 4.793 & 1.823 & 3.062 & 1.440 & 2.953 & 1.439 \\
 & 336 & 1.398          & 0.869          & 1.574 & 0.937 & 1.545 & 0.928  & 1.474 & 0.911 & 1.822 & 1.041  & 1.976 & 1.101 & 4.313 & 1.740 & 3.111 & 1.467 & 2.923 & 1.428 \\
 & 720 & 1.606          & 0.957          & 1.743 & 1.005 & 1.749 & 1.004  & 1.635 & 0.975 & 1.836 & 1.056  & 1.947 & 1.084 & 3.976 & 1.662 & 3.069 & 1.456 & 2.975 & 1.440 \\
 & Avg & \textbf{1.265} & \textbf{0.803} & 1.430 & 0.874 & 1.428 & 0.873  & 1.347 & 0.851 & 1.705 & 0.996  & 1.809 & 1.034 & 4.627 & 1.790 & 3.275 & 1.503 & 2.855 & 1.410 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Nordpool}} 
 & 96  & 0.554          & 0.545          & 0.631 & 0.591 & 0.638 & 0.594  & 0.629 & 0.595 & 0.789 & 0.694  & 0.888 & 0.737 & 2.247 & 1.190 & 1.889 & 1.116 & 1.876 & 1.102 \\
 & 192 & 0.613          & 0.582          & 0.707 & 0.636 & 0.704 & 0.633  & 0.687 & 0.635 & 0.734 & 0.673  & 1.031 & 0.798 & 2.400 & 1.240 & 2.052 & 1.141 & 2.055 & 1.140 \\
 & 336 & 0.594          & 0.581          & 0.674 & 0.626 & 0.679 & 0.627  & 0.678 & 0.635 & 0.756 & 0.680  & 0.860 & 0.727 & 2.484 & 1.267 & 2.022 & 1.121 & 2.175 & 1.175 \\
 & 720 & 0.577          & 0.578          & 0.660 & 0.626 & 0.674 & 0.632  & 0.677 & 0.638 & 0.812 & 0.707  & 0.938 & 0.758 & 2.579 & 1.385 & 1.641 & 1.013 & 2.161 & 1.178 \\
 & Avg & \textbf{0.585} & \textbf{0.572} & 0.668 & 0.620 & 0.674 & 0.6215 & 0.668 & 0.626 & 0.773 & 0.689  & 0.929 & 0.755 & 2.428 & 1.271 & 1.901 & 1.098 & 2.067 & 1.149 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Caiso}} 
 & 96  & 0.210          & 0.290          & 0.246 & 0.328 & 0.243 & 0.329  & 0.247 & 0.329 & 0.499 & 0.514  & 0.664 & 0.607 & 1.641 & 0.902 & 1.229 & 0.808 & 1.226 & 0.790 \\
 & 192 & 0.285          & 0.349          & 0.320 & 0.382 & 0.317 & 0.382  & 0.315 & 0.380 & 0.539 & 0.534  & 0.835 & 0.671 & 1.801 & 0.945 & 1.269 & 0.820 & 1.317 & 0.822 \\
 & 336 & 0.334          & 0.384          & 0.377 & 0.421 & 0.376 & 0.421  & 0.365 & 0.413 & 0.634 & 0.583  & 0.795 & 0.655 & 2.076 & 1.026 & 1.442 & 0.858 & 1.401 & 0.846 \\
 & 720 & 0.436          & 0.444          & 0.525 & 0.509 & 0.547 & 0.523  & 0.494 & 0.499 & 0.807 & 0.667  & 0.884 & 0.705 & 2.361 & 1.230 & 1.560 & 0.891 & 1.735 & 0.942 \\
 & Avg & \textbf{0.316} & \textbf{0.367} & 0.367 & 0.41  & 0.371 & 0.414  & 0.355 & 0.405 & 0.620 & 0.5745 & 0.795 & 0.660 & 1.970 & 1.026 & 1.375 & 0.844 & 1.420 & 0.85\\ 
 
\midrule

%\multicolumn{2}{c|}{Average}& \textbf{0.308} & \textbf{0.305} 0.371 &0.367 &0.385  &0.376&0.511 &0.472 &0.687 &0.559 &0.674 &0.522 &0.912 &0.665 &1.137 &0.712 &1.850 &0.967 &1.888 &0.974  \\

% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:few_shot_10}
}
% \end{adjustwidth}
\vskip 0.1in
%\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/few_shot_5.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 5\% data. All the results are averaged from 4 different prediction lengths $O \in {96, 192, 336, 720}$.A lower MSE indicates better performance, and the best results are highlighted in bold. ’-’ means that 5\% time series is not sufficient to constitute a training set.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}

\toprule
\multicolumn{2}{c|}{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c|}{Reformer}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\
\midrule
\multirow{5}{*}{\rotatebox{90}{ETTm1}} 

&96  & 0.332  & 0.369   & 0.399 & 0.414 & 0.386 & 0.405 & 0.332 & 0.374 & 0.628 & 0.544 & 0.726 & 0.578 & 1.13  & 0.775 & 1.446 & 0.928 & 1.234 & 0.798 \\
&192 & 0.376  & 0.398   & 0.441 & 0.436 & 0.44  & 0.438 & 0.358 & 0.39  & 0.666 & 0.566 & 0.75  & 0.591 & 1.15  & 0.788 & 1.519 & 0.962 & 1.287 & 0.839 \\
&336 & 0.425  & 0.423   & 0.499 & 0.467 & 0.485 & 0.459 & 0.402 & 0.416 & 0.807 & 0.628 & 0.851 & 0.659 & 1.198 & 0.809 & 1.774 & 1.032 & 1.288 & 0.842 \\
&720 & 0.486  & 0.458   & 0.767 & 0.587 & 0.577 & 0.499 & 0.511 & 0.489 & 0.822 & 0.633 & 0.857 & 0.655 & 1.175 & 0.794 & 1.647 & 0.994 & 1.247 & 0.828 \\
&Avg & \textbf{0.405}  & \textbf{0.412}   & 0.526 & 0.476 & 0.472 & 0.45  & 0.400 & 0.417 & 0.73  & 0.592 & 0.796 & 0.62  & 1.163 & 0.791 & 1.597 & 0.979 & 1.264 & 0.826 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Electricity}} 
&96  & 0.147  & 0.246   & 0.145 & 0.244 & 0.143 & 0.241 & 0.15  & 0.251 & 0.235 & 0.322 & 0.297 & 0.367 & 1.265 & 0.919 & 0.816 & 0.687 & 1.414 & 0.855 \\
&192 & 0.164  & 0.262   & 0.163 & 0.26  & 0.159 & 0.255 & 0.163 & 0.263 & 0.247 & 0.341 & 0.308 & 0.375 & 1.298 & 0.939 & 0.778 & 0.666 & 1.24  & 0.919 \\
&336 & 0.189  & 0.285   & 0.183 & 0.281 & 0.179 & 0.274 & 0.175 & 0.278 & 0.267 & 0.356 & 0.354 & 0.411 & 1.302 & 0.942 & 0.889 & 0.717 & 1.253 & 0.921 \\
&720 & 0.242  & 0.334   & 0.233 & 0.323 & 0.233 & 0.323 & 0.219 & 0.311 & 0.318 & 0.394 & 0.426 & 0.466 & 1.259 & 0.919 & 1.251 & 0.912 & 1.249 & 0.921 \\
&Avg & \textbf{0.185} & \textbf{0.281} & 0.181 & 0.277 & 0.178 & 0.273 & 0.176 & 0.275 & 0.266 & 0.353 & 0.346 & 0.404 & 1.281 & 0.929 & 0.934 & 0.746 & 1.289 & 0.904 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}} 
&96  & 0.413  & 0.279   & 0.404 & 0.286 & 0.419 & 0.298 & 0.427 & 0.304 & 0.67  & 0.421 & 0.795 & 0.481 & 1.557 & 0.821 & 1.149 & 0.599 & 1.586 & 0.841 \\
&192 & 0.425  & 0.287   & 0.412 & 0.294 & 0.434 & 0.305 & 0.447 & 0.315 & 0.653 & 0.405 & 0.837 & 0.503 & 1.596 & 0.834 & 1.247 & 0.657 & 1.602 & 0.844 \\
&336 & 0.440  & 0.297   & 0.439 & 0.31  & 0.449 & 0.313 & 0.478 & 0.333 & 0.707 & 0.445 & 0.867 & 0.523 & 1.621 & 0.841 & 1.531 & 0.799 & 1.668 & 0.868 \\
&720 & -      & -       & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     \\
&Avg & \textbf{0.426}  & \textbf{0.288}   & 0.418 & 0.296 & 0.434 & 0.305 & 0.45  & 0.317 & 0.676 & 0.423 & 0.833 & 0.502 & 1.591 & 0.832 & 1.309 & 0.685 & 1.618 & 0.851 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}}
&96  & 0.161  & 0.205   & 0.171 & 0.224 & 0.175 & 0.23  & 0.184 & 0.242 & 0.229 & 0.309 & 0.227 & 0.299 & 0.497 & 0.497 & 0.356 & 0.408 & 0.406 & 0.435 \\
&192 & 0.219  & 0.256   & 0.23  & 0.277 & 0.227 & 0.276 & 0.228 & 0.283 & 0.265 & 0.317 & 0.278 & 0.333 & 0.62  & 0.545 & 0.489 & 0.479 & 0.446 & 0.45  \\
&336 & 0.289  & 0.308   & 0.294 & 0.326 & 0.286 & 0.322 & 0.279 & 0.322 & 0.353 & 0.392 & 0.351 & 0.393 & 0.649 & 0.547 & 0.517 & 0.482 & 0.465 & 0.459 \\
&720 & 0.361  & 0.361   & 0.384 & 0.387 & 0.366 & 0.379 & 0.364 & 0.388 & 0.391 & 0.394 & 0.387 & 0.389 & 0.57  & 0.522 & 0.465 & 0.463 & 0.471 & 0.468 \\
&Avg & \textbf{0.258}  & \textbf{0.283}   & 0.269 & 0.303 & 0.263 & 0.301 & 0.263 & 0.308 & 0.309 & 0.353 & 0.31  & 0.353 & 0.584 & 0.527 & 0.457 & 0.458 & 0.447 & 0.453 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Wind}}
&96  & 1.131  & 0.735   & 1.109 & 0.739 & 1.139 & 0.754 & 1.058 & 0.720 & 1.503 & 0.922 & 1.609 & 0.948 & 5.978 & 1.939 & 4.573 & 1.661 & 2.290 & 1.244 \\
&192 & 1.150  & 0.757   & 1.417 & 0.873 & 1.434 & 0.873 & 1.328 & 0.846 & 1.682 & 0.982 & 1.824 & 1.014 & 4.340 & 1.665 & 4.390 & 1.665 & 2.575 & 1.312 \\
&336 & 1.398  & 0.869   & 1.595 & 0.947 & 1.614 & 0.954 & 1.484 & 0.917 & 1.833 & 1.040 & 2.069 & 1.094 & 3.662 & 1.540 & 3.620 & 1.539 & 2.715 & 1.350 \\
&720 & 1.606  & 0.957   & 1.755 & 1.008 & 1.767 & 1.012 & 1.712 & 0.994 & 1.944 & 1.075 & 2.069 & 1.096 & 2.751 & 1.343 & 2.806 & 1.368 & 2.797 & 1.372 \\
&Avg & \textbf{1.321}  & \textbf{0.830}   & 1.469 & 0.892 & 1.489 & 0.898 & 1.396 & 0.869 & 1.741 & 1.005 & 1.893 & 1.038 & 4.183 & 1.622 & 3.847 & 1.558 & 2.594 & 1.320 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Nordpool}}
&96  & 0.554  & 0.545   & 0.668 & 0.610 & 0.687 & 0.619 & 0.659 & 0.612 & 0.936 & 0.751 & 0.952 & 0.763 & 4.267 & 1.690 & 2.675 & 1.335 & 1.929 & 1.121 \\
&192 & 0.613  & 0.582   & 0.729 & 0.647 & 0.766 & 0.661 & 0.728 & 0.650 & 0.923 & 0.752 & 1.052 & 0.809 & 3.568 & 1.535 & 2.195 & 1.202 & 2.015 & 1.149 \\
&336 & 0.719  & 0.647   & 0.721 & 0.649 & 0.766 & 0.665 & 0.728 & 0.659 & 0.959 & 0.775 & 1.069 & 0.815 & 2.552 & 1.287 & 1.976 & 1.133 & 2.012 & 1.149 \\
&720 & 0.728  & 0.658   & 0.724 & 0.660 & 0.789 & 0.680 & 0.725 & 0.662 & 0.999 & 0.787 & 0.904 & 0.750 & 2.246 & 1.206 & 1.836 & 1.083 & 2.004 & 1.150 \\
&Avg & \textbf{0.654}  & \textbf{0.608}   & 0.711 & 0.642 & 0.752 & 0.656 & 0.71  & 0.646 & 0.954 & 0.766 & 0.994 & 0.784 & 3.158 & 1.430 & 2.171 & 1.188 & 1.99  & 1.142 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Caiso}}
&96  & 0.209  & 0.289   & 0.262 & 0.344 & 0.269 & 0.357 & 0.262 & 0.346 & 0.515 & 0.529 & 0.636 & 0.595 & 1.485 & 0.879 & 1.452 & 0.875 & 1.290 & 0.812 \\
&192 & 0.285  & 0.347   & 0.330 & 0.393 & 0.323 & 0.393 & 0.327 & 0.394 & 0.579 & 0.562 & 0.680 & 0.610 & 1.721 & 0.949 & 1.586 & 0.902 & 1.405 & 0.850 \\
&336 & 0.348  & 0.386   & 0.388 & 0.435 & 0.379 & 0.433 & 0.378 & 0.431 & 0.651 & 0.601 & 0.699 & 0.613 & 1.829 & 0.977 & 1.643 & 0.905 & 1.465 & 0.876 \\
&720 & 0.432  & 0.442   & 0.564 & 0.533 & 0.558 & 0.539 & 0.560 & 0.534 & 0.866 & 0.703 & 0.901 & 0.712 & 2.106 & 1.057 & 1.975 & 1.006 & 1.573 & 0.909 \\
&Avg & \textbf{0.319}  & \textbf{0.366}   & 0.386 & 0.426 & 0.382 & 0.431 & 0.382 & 0.426 & 0.653 & 0.599 & 0.729 & 0.633 & 1.785 & 0.966 & 1.664 & 0.922 & 1.433 & 0.862\\

\midrule


%\multicolumn{2}{c|}{Average} & \textbf{0.316}  & \textbf{0.314} & 0.377 &0.375  &0.392 &0.383  &0.483 &0.445 &0.537 &0.480 &0.697 &0.537 &0.909 &0.675 &1.341 &0.789 &1.878 &0.994 &1.819 &0.966\\
% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:few_shot_5}
}
% \end{adjustwidth}
\vskip 0.1in
%\vskip -0.1in
\end{sc}
\end{table*}
%}
